Conformance Testing of Relational DBMS Against SQL Specifications

A Relational Database Management System (RDBMS) is one of the fundamental software that supports a wide range of applications, making it critical to identify bugs within these systems. There has been active research on testing RDBMS, most of which employ crash or use metamorphic relations as the oracle. Although existing approaches can detect bugs in RDBMS, they are far from comprehensively evaluating the RDBMS's correctness (i.e., with respect to the semantics of SQL). In this work, we propose a method to test the semantic conformance of RDBMS i.e., whether its behavior respects the intended semantics of SQL. Specifically, we have formally defined the semantics of SQL and implemented them in Prolog. Then, the Prolog implementation serves as the reference RDBMS, enabling differential testing on existing RDBMS. We applied our approach to four widely-used and thoroughly tested RDBMSs, i.e., MySQL, TiDB, SQLite, and DuckDB. In total, our approach uncovered 19 bugs and 11 inconsistencies, which are all related to violating the SQL specification or missing/unclear specification, thereby demonstrating the effectiveness and applicability of our approach.

==> 3-semantics-old.tex <==
\section{Formal Semantics for SQL}
\label{sec:semantics}


\begin{table}[t]   
\begin{center}   
\caption{Symbol notations}
\label{table:basic} 
\small
\begin{tabular}{rl}   
\toprule   
Symbol & Description \\      
% \multirow{5}*{Schema}&$\mathbb{S}$ & schema  \\
% &$\mathbb{D}$ & database  \\ 
% &$\mathbb{T}$ & table  \\ 
% &n & names(table name and column name)  \\ 
% &v & the value of the attribute in the table \\ 
% &c & constants \\
% &t & expression \\
% &$\overline t(t_1,...,t_k)$ & bags of expression \\
% &$\hat t(t_1,...,t_k)$ & sets of expression \\
% &Z & set of all integers \\
% &$\pi$ &  Get the columns in the data table \\
% &$\sigma$ &  Get the rows in the data table \\
\midrule
\texttt{T} & A table instance \\
% \multirow{2}*{T} & a table instance \\
% &contains attributes and values T=$(\overline{\beta},\overline{\alpha})$  \\ 
$ \alpha$ & A data record in a table  \\ 
$ \widehat{\alpha}$ & Bags of data records  \\
$ \beta$ & An attribute in a table  \\
$ \widehat{\beta}$ & Bags of attributes  \\
$ \Theta $ & An expression\\
 \texttt{T}.$\beta_i$ & The i$_{th}$ attribute in \texttt{T}  \\
\texttt{T}.$\overline{\beta}$ & All attributes in  \texttt{T}\\
% &L(T) & the bag of all attributes of the data table\ T  \\
% &V(T) & the bag of all datas of the data table\ T  \\
$ \pi_{\beta}(\texttt{T})$ & Data projection on attribute $\beta$  \\
$\sigma_{\Theta}(\texttt{T})$ & Data selection on expression $\Theta$  \\
$ \xi_{\alpha}(\texttt{T})$ & The multiplicity of data record $\alpha$ in table \texttt{T}\\
$ \xi_{\beta}(\texttt{T})$ & The multiplicity of 
attribute $\beta$ in table \texttt{T} \\
% $ str$ & A string \\
% % $ l$ & The length of a  string \\
% $STR$ & A string list \\
% $ index$ & The subscript of a list or string  \\
$ [a,...,a]_n$ & A list of element a with length n   \\
% $\circ$ & 连接操作   \\
$\bowtie$ & Data join operation \\
$\times$ & Cartesian product operation   \\
% $max(a_1,a_2)$ &The maximum value in $a_1 $and $a_2 $    \\
% $min(a_1,a_2)$ &The minimum value in $a_1 $and $a_2 $    \\
% $str(n)$ &The string representation of the numeric type n   \\
% $num(s)$ &The numeric representation of the string type s    \\
% $type(a)$ &The data type of a    \\
% $ascii(a)$ &The ASCII code value of a    \\
% $ [a,...,a]_n$ & A data list of length n and all elements are a   \\
% $\circ$ & Concatenate operation on two data records   \\
% $|\ \ |$ & the length of the value \\
% $null$ & unknown\ data \\
% $\wedge$ & and \\
% $\vee$ & or \\
% $\neg$ & not \\
% $c$ & constant,include\ integer\ and\ float \\
% $boolean$   & TRUE\ $|$\ FALSE \\
% $str$ &  String\ type\\
% $char$ &  character\ type\\
\bottomrule  
\end{tabular}   
\end{center}   
\end{table}



\input{semantic}

% This work requires the formulation of semantics based on the functional descriptions of keywords in the SQL specification, necessitating the establishment of preconditions and postconditions for various SQL operations.

% In this section, we first presented some fundamental definitions, including symbols for databases, tables, attributes, and data, as well as the definitions of basic operations for retrieval. Building upon these definitions, we then established the formal semantics for keywords.

%在这部分中，我们首先介绍了一些基础定义，包括一些对数据库，表，属性，数据的符号定义和对一些检索时的基本操作的定义。在这些定义的基础上，我们定义了关键字的形式化语义。
% \subsection{basic notations}

%在基础定义部分中，我们首先定义了数据库模式，数据库和表的抽象符号，之后我们定义了对表的两项基本操作，取行和取列，我们可以通过这两项操作定位到一个具体的数据。
 
% we initially defined abstract symbols for database schema, database, and tables. Subsequently, we introduced two fundamental operations on tables, namely, retrieving rows and retrieving columns. These operations allow us to locate specific data within a table.
%接下来我们对数据库实例进行了定义，首先定义了数据库，表，表中数据和列属性的实例，之后在取行和取列操作的基础上结合表，属性的实例进行了更具体的定义。
% we proceeded with the definition of database instances. 
% we start by defining instances of databases, tables, data within the tables, and attributes of columns. Building upon the operations of data projection and selection, we further refine the definitions retrieving rows and columns by incorporating concrete instances of tables and attributes. We use $\xi$ express the data or attribute number in the table.
%SQL语句的输入来自表中的数据，但在处理SQL语句的过程中，我们需要处理表达式，我们定义了表达式的种类，首先是数据，我们结合SQL Specification和我们的Prolog语义实现给出了四种数据类型的数据定义，分别是常数(包含整数和浮点数)，布尔类型，字符串类型和字符类型。其次是null的语义，null在SQL中代表未知，是SQL执行过程中需要单独处理的数据类型。第三种就是各种逻辑表达式，我们在下面的的关键字语义中会对各种逻辑运算符进行详细的定义，在基础定义中，我们引入了与，或，非的基本运算。

% % In the process of handling SQL statements, the inputs are derived from the data within the tables. 
% To effectively process SQL statements, we also need to handle expressions. For this purpose, we have defined various types of expressions. First, we have data expressions, which include four data types based on SQL Specification. These data types are constants (including integers and floating-point numbers), booleans, strings, and characters.We use $v$ express the value of the data and use $len()$ express the length of the value. 
% Next, we have defined the semantics for null values. 
% % In SQL, null represents unknown data and requires special handling during the execution process. 
% Lastly, we have addressed various logical expressions. 
% % Detailed definitions for logical operators will be presented in the subsequent section on keyword semantics. 
% % In the foundational definitions, 
% We have introduced basic operations such as $\wedge$, $\vee$, and $\neg$.These three symbols represent set operations of intersection, union, and complement.

% In the context of basic semantics for databases, we initially define the database schema, symbols representing databases, and data tables. On the basis of these three definitions, we also defined constants, lists, sets, and operations for data retrieval such as getting the rows or columns in the data table. The second part in Table I pertains to the definition and manipulation of database instances, which represent the actual data present in the data tables. In this section of the definition, we combine the concrete data instances with the foundational definitions described earlier to facilitate the process of writing the semantics for specific keywords.Lastly, Table II covers the fundamental definition of conditional statements for decision-making processes.In the process of SQL execution, the results obtained are not limited to specific single or multiple data records. They can also include other data types such as boolean data types and NULL values. Additionally, for the convenience of representing semantics, we introduce basic operations for sets, including union, intersection, and complement.

% \begin{framed}
% \leftline{$ \Theta(expression): \\ $}
% $$ \left\{
% \begin{aligned}
% &v,&t&he\ value\ of\ the\ data\ \\
% nu&ll,&u&nknown\ data \\
% logic\ ex&pression,&\Theta&\wedge \Theta\ |\ \Theta \vee \Theta\ | \neg \Theta \\
% \end{aligned}
% \right.
% $$
% $$ v=\left\{
% \begin{aligned}
% c,\    & constant,include\ integer\ and\ float \\
% boolean,\   & TRUE\ |\ FALSE \\
% str,\ &  String\ type\\
% char,\ &  character\ type\\
% \end{aligned}
% \right.
% $$
% % \leftline{$ P(predicate): \\ $}
% % $$ P(t_1,...,t_k)=\left\{
% % \begin{aligned}
% % T,\    & (P(t_1,...,t_k))\wedge \\
% %      &  (\forall i \in (1, ...,k),\ t_i != NULL)\\
% % F,\   & (!(P(t_1,...,t_k)))\wedge \\
% %      &  (\forall i \in (1, ...,k),\ t_i != NULL)\\
% % U,\ & \exists i \in (1, ...,k),\ t_i = NULL \\
% % \end{aligned}
% % \right.
% % $$
% % $$ t\ IN\ \overline{t}=\left\{
% % \begin{aligned}
% % T,\    &  \exists i \in (1, ...,k),\ t = t_i \\
% % F,\   &  \forall i \in (1, ...,k),\ t != t_i\\
% % U,\ & (\exists i \in (1, ...,k),\ t_i = NULL)\wedge\\
% % & (\forall i \in (1, ...,k),(t !=t_j) \wedge (t_j!=NULL)) \\
% % \end{aligned}
% % \right.
% % $$
% \end{framed}

% \subsection{keyword semantic}
% In the section of keyword semantics, we implemented it based on SQL Specification. 

% Referring to the method proposed by Hoare\cite{b41}, a pair of formulas are placed before and after the corresponding program segment, which are called the precondition and postcondition of the program segment respectively.\\
We first define the denotational semantics for SQL, according to the SQL specification documented in ISO/IEC 9075:2016~\cite{iso-iec-9075-2016}.  
Table~\ref{table:basic} lists the basic notations used in our semantic definitions. We use \texttt{T}, $\alpha$, $\beta$ to represent a table, a data record in a table and an attribute of a table, respectively. 
$ \widehat{\alpha}$ and $ \widehat{\beta}$ represent the bags of data records and bags of attributes, as we follow the ISO standard and define the bag semantics of SQL.  
$\Theta$ denotes expressions, including logical expressions, numeric expressions, constant values and function operations defined in SQL. 
We use $\pi$, $\sigma$ and $\xi$ to represent the data projection operation, data selection operation and the multiplicity calculation on the occurrences of a data records or attributes, respectively. 
% \tcl{
The symbols $\bowtie$ and $\times$ are used to represent the join operation and the Cartesian product operation on two data records, respectively. Additionally, this work uses $[a,...,a]_n$ to denote a list of n items of a (which can be variable  or constants). 
\begin{comment}
The functions $max(a_1, a_2)$ and $min(a_1, a_2)$ are used to perform operations that find the maximum or minimum value between $a_1$ and $a_2$. The operations $str(n)$ and $num(s)$ are used to convert between numeric types and string types. Lastly, the functions $type(a)$ and $ascii(a)$ are used to determine the data type and ASCII value of the data $a$, respectively.    
\end{comment}
% }

% As there are various functions involve string calculation, we use $str$, $STR$ and $index$ to represent a string, a string list and the subscript of a list or string. 

% We adopt the format of the Hoare triple~\cite{hoare2003verifying}, as shown in Formula~(\ref{eq:hoaretriple}), to formalize the SQL semantics.  In the Hoare triple format, \textit{P} and \textit{Q} are assertions in predicate logic, where \textit{P} represents the precondition and \textit{Q} the postcondition, while \textit{C} is the command. 
% If the precondition \textit{P} evaluates to true, then executing the command \textit{C} establishes the postcondition \textit{Q}. 


% \begin{equation}
% \label{eq:hoaretriple}
%  \{P\} C \{Q\}\\    
% \end{equation}

% If the condition pre is established before the execution of program P (the environment at that time meets pre), the condition post must be established in the environment when the execution of program P terminates.

We manually analyze the semantics of keywords in the SQL specification and defined the denotational semantics for 138 SQL keywords or features related to query functionality in the SQL specification. Due to space limitations, we present a selective list of SQL semantics (grammar in Figure~\ref{fig:wenfa} and semantic rules in Figure~\ref{fig:semantic1}). 
% \tcl{
The full set of semantic rules can be found in the Appendix. %~\ref{appendix}.
% s}

\tcl{Based on the different return values of SQL functions, we have categorized the semantics of SQL into the semantics of SQL expressions and the semantics of SQL keywords. The former includes three types of expressions. In Figure~\ref{fig:semantic1}, we have demonstrated the semantics of Boolean-type expressions represented by logical expressions (Semantics 1-9), where we use the $\mathcal{B}$ function to denote the mapping from Boolean value expressions to Boolean values. Additionally, we have shown the semantics of numeric-type expressions represented by arithmetic expressions (Semantics 10-15), where we use the $\mathcal{N}$ function to represent the mapping from numeric expressions to numeric values. Moreover, we have also defined the semantics of SQL functions that return string types.}

\tcl{The semantics of SQL keywords, which may cause changes in the state of tables in the database, are categorized based on specific SQL functions into SQL semantics from table instance to table instance and SQL semantics from expressions to table instance. The semantics of the join operation (Semantics 16-18) shown in Figure~\ref{fig:semantic1} belong to the SQL semantics from table instance to table instance. The input of this operation includes one or more table instances and the operation type, with the output being a new table instance. In this context, $L$ represents the list of table instances to be processed, and $OP$ represents the type of operation performed. The $\{L, OP\}$ structure represents the input of these SQL functions. The function $\mathcal{C}$ describes the process $\{L, OP\} \mapsto T$.}

\tcl{The semantics of the second type of SQL keywords include from, where, on, select, group by, having, and order by. The input for these semantic functions is their corresponding SQL expressions, and the output is $(S, T)$, a form of table state tuple. $S$ represents the set of database tables that are of interest during execution, indicating that not all tables are relevant when performing certain SQL functions. $S$ is the set of tables that actually participate in or are affected during the execution. $T$ represents the temporary table obtained after execution, typically generated after query operations to store the temporary dataset of query results. The function $H$ describes the process $Expression \mapsto (S, T)$.}

\tcl{Based on the semantics of these keywords and functions, we define the composite semantics of SQL language to represent the semantics of a complete SQL statement. The input of the composite semantics is a SQL statement, and the output is a $(S, T) $. We first introduced the combination rules of different types of keyword semantics (Semantics 30), and then we combined specific keyword semantics based on these rules (Semantics 31).}

% We conducted a statistical analysis of the keywords documented in the SQL specification, and identified a total of 138 keywords. 
% We have defined the semantics for each of these keywords.

% Due to space limitations, we selectively present the semantic rules in Figure~\ref{fig:semantic1}, and the full set of semantic rules can be found in our technical report~\cite{technicalReport}.

% We provide denotational semantics, where we only  formally specify the effects of certain operations/keywords, rather than encoding the procedures of how to conduct the computations. 
% We have categorized the basic semantic rules for keywords into the following groups, i.e., basic query expressions, join operations, logical operations, aggregation operations, group operations, collection operations, and function operations.

% Building upon the foundation of individual keyword semantics, we have defined the composite semantics for SQL queries.

% Building upon the foundation of keyword semantics, we defined the composite semantics for SQL queries. 
% \tcl{
% Based on the foundation of encompassing all the previously mentioned keyword semantics, these composite statement forms ensure both brevity and conciseness in the statements.
% %On the foundation of covering all the above-mentioned keyword semantics, these composite statement forms ensure brevity and conciseness of the statements. 
% For instance, in Statement 5 in Figure~\ref{fig:semantic1}, which addresses Aggregation Operations, operations such as \texttt{GROUP BY} and \texttt{HAVING} are typically used concurrently.
% %For instance, in Statement 4 concerning Aggregation Operation, operations such as \texttt{GROUP BY} and \texttt{HAVING} are generally used concurrently. 
% Therefore, we have integrated these three functionalities into a single, composite statement.
% Here, $\Theta$ encompasses all Logical Operation keywords and Function Operation keywords, offering a comprehensive and streamlined representation.
% }
% Figure~\ref{fig:semantic1} illustrates seven types of composite semantics we defined, the full list of composite semantics can be found in our technical report~\cite{technicalReport}. 
% The criteria for selecting which composite semantics to define are (1) covering various types of adjacent keywords and (2) ensuring conciseness of composite statements by removing redundant and repetitive parts. For instance, in CQ5 in Figure~\ref{fig:semantic1}, the statement involves group operations, where the SQL group operation typically uses the \texttt{group by} and \texttt{having} keywords together. Therefore, we have combined these two keywords and retained only the \texttt{select} and \texttt{from} keywords to ensure the simplicity of the statement while maintaining grammatical correctness. Additionally, the symbol $\Theta$ represents all logical and functional keywords, which appear in logical expressions and are often used as filtering conditions following keywords such as \texttt{where} or \texttt{having} in SQL statements. 

%我们的形式化语义并没有将每个我们支持的关键字的语义都呈现出来，如算术运算（+、-、*、/）、比较运算（>、<）以及位运算（&、|）等，这些运算在更高层次的编程语言或者其他计算领域中都有详细的定义和广泛的应用。因此，我们的形式化语义不包含这些基本运算符的具体运算规则和用法。另外，有一些语义相同的关键字我们进行了合并，比如UPPER和UCASE函数，语义都是将字符串中的小写字母转化为大写字母。
% \tcl{In our formal semantics, we have not explicitly delineated the semantics of every supported keyword, particularly for operations such as arithmetic operations ($+, -, *, /$), comparison operations ($>, <$), and bitwise operations ($\&, |$). These operations have been comprehensively defined and are widely applied across higher-level programming languages and various computational domains. Consequently, our formal semantics omits the specific operational rules and usages of these fundamental operators.}

% \tcl{Furthermore, we have consolidated keywords with identical semantics to streamline our presentation and reduce redundancy. For example, the functions UPPER and UCASE, which both transform lowercase letters in a string to uppercase, have been merged under a unified semantic representation in our documentation. This approach not only maintains the integrity of our formal semantics but also ensures clarity and conciseness in our linguistic expressions.}
% \begin{spacing}{0.2}


% \end{spacing}

%在关键字语义的基础上，我们给出了四种常见语句模式的组合语义，这些组合语义包含的关键字有select，from，where，group by，order by，having，聚合函数


% These composite semantics encompass keywords such as select, from, where, group by, order by, having, and aggregate functions.
%这些组合语句形式在覆盖了上面所有的关键字语义的基础上，保证了语句的简洁，比如语句4中Aggregation Operation，GROUP BY和HAVING操作一般会同时使用，所以我们将这三个功能整合到了一条组合语句中，\Theta包含了所有的Logical operation和Function operation。

% \begin{spacing}{0.05}
% {\scriptsize
% \begin{framed}
% \leftline{$ T_s:\pi_{\overline{\beta}}(T)$}
% ~\\
% \leftline{
% $
% \begin{aligned}
% T_w:&(\forall \alpha \in \sigma_\Theta (T),\alpha \in T_w) 
%  \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_w)\\
% &\wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_w))
% \end{aligned}
% $
% }
% \leftline{$ T_{sw}:\pi_{\overline{\beta}}(T_s)$}
% \\ \hspace*{\fill} \\
% \leftline{1. SELECT $T.\overline{\beta}$ FROM T \\ }
% \\ \hspace*{\fill} \\
% $\frac{\left\{T\right\}\ FROM\ \left\{T\right\},\ \left\{T\right\}\ SELECT\ \overline{\beta}\  \left\{T_{s}\right\}}{\left\{T\right\}\ FROM;\ SELECT\ \overline{\beta}   \left\{T_{s}\right\}}$
% \\ \hspace*{\fill} \\
% ~\\
% \leftline{2. SELECT $T.\overline{\beta}$ FROM T WHERE $\Theta$ \\ }
% \\ \hspace*{\fill} \\
% $\frac{\left\{T\right\}\ FROM\ \left\{T\right\},\ \left\{T\right\}\ WHERE\ \Theta\  \left\{T_w\right\},\left\{T_w\right\}\ SELECT\ \overline{\beta}\   \left\{T_{sw}\right\}}{\left\{T\right\}\ FROM;\ WHERE\ \Theta;\ SELECT\ \overline{\beta}\    \left\{T_{sw}\right\}}$
% \\ \hspace*{\fill} \\
% ~\\
% \leftline{3. SELECT $\beta_1$, Aggregation Operation ($T.\beta_2$) FROM T \\}
% \leftline{GROUP BY $\beta_1$ HAVING $\Theta$ \\ }
% ~\\
% $\frac{\left\{T\right\}\ FROM\ \left\{T_1\right\},\ \left\{T_1\right\}\ GROUP\ BY\ \left\{T_2\right\},\ \left\{T_2,\beta_2\right\}\ Agg\ \left\{x_{agg}\right\},\ \ }{\left\{T,\beta_2\right\}\ FROM;\ GROUP\ BY;\ AGG     \left\{x_{agg}\right\}}$
% \\ \hspace*{\fill} \\
% $\frac{\left\{T_2,\beta_1,\beta_2,x_{agg}\right\}\ SELECT\ \left\{T_3\right\},\ \left\{T_3,\Theta\right\}\ HAVING\ \left\{T_4\right\}\ }{\left\{T_2,\beta_1,\beta_2,x_{agg}\right\}\ SELECT;\ HAVING;\     \left\{T_4\right\}}$
% \\ \hspace*{\fill} \\
% ~\\
% \leftline{4. SELECT $T.\beta_1$ FROM T ORDER BY $\beta_1$ ASC/DESC\\}
% ~\\
% $\frac{\left\{T\right\}\ FROM\ \left\{T_1\right\},\ \left\{T_1,\beta_1\right\}\ SELECT\ \left\{T_2\right\},\left\{T_2,\beta_1\right\}\ ORDER\ BY \left\{T_3\right\} \ }{\left\{T,\beta_1\right\}\ FROM;\ SELECT;\ ORDER\ BY;\left\{T\right\} }$
% % \\ \hspace*{\fill} \\
% % $\frac{\left\{T_2,\beta_1\right\}\ ORDER\ BY \left\{T_3\right\} }{\left\{T_2,\beta_1\right\}\ ORDER\ BY;\     \left\{T_3\right\}}$
% \\ \hspace*{\fill} \\
% \\ \hspace*{\fill} \\
% \leftline{5. SELECT $T\-1.\overline{\beta}$ FROM $T\_1$ Join Operation $T\_2$ \\ }
% $\frac{\left\{T_1,T_2\right\}\ JOIN\ Operation\ \left\{T\right\},\left\{T\right\}\ FROM\ \left\{T\right\},\ \left\{T\right\}\ SELECT\ \overline{\beta}\  \left\{T_{s}\right\}}{\left\{T\right\}\ JOIN\ Operation;\ FROM;\ SELECT\ \overline{\beta}   \left\{T_{s}\right\}}$
% \\ \hspace*{\fill} \\
% \\ \hspace*{\fill} \\
% \leftline{6. $T_1,T_2$ Collection Operation $T$ \\}
% $\{T_1,T_2\}\ Collection\ Operation\ \{T\}$
% \end{framed}
% }
% \end{spacing}
% \begin{figure*}
% \begin{framed}
% \leftline {\textbf{KEYWORD}\\}
% \leftline {\textbf{Query expression}\\}
% \leftline {1. FROM: from T\\}
% $\left\{T\right\}\ FROM\ \left\{T_1\right\}$
% \\ \hspace*{\fill} \\
% \leftline {2. SELECT: select\ $T.\overline{\beta}$\\}
% $\left\{T,\overline{\beta}\right\}\ SELECT\ \left\{T_1|T_1=\left\{\pi_{\overline{\beta}}(T)\right\}\right\}$
% \\ \hspace*{\fill} \\
% \leftline {3. WHERE: where\ $\Theta$\\}
% $\left\{T,\Theta\right\}\ WHERE$
% $\left\{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1)\\ \right.$
% $\left. \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)\right.$
% $\left. \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\right\}$
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Collection operation}\\}
% \leftline{4. UNION: T1 union T2 \\ }
% $
% \left\{T_{1}, T_{2}\right\}\ UNION$
% \\
% $\left\{T | (\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2, \alpha_{1} , \alpha_{2} \in T) \right.$
% \\
% $\left. \wedge(\forall \alpha_{3} \in T,(\alpha_{3} \in T_1)\vee(\alpha_{3} \in T_2))\right.$
% $ \left. \wedge (\forall \alpha_4 \in T,\ \xi_{\alpha_4}(T)=1)\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{5. INTERSECT: T1 intersect T2 \\ }
% $\left\{T_{1}, T_{2}\right\}\ INTERSECT$
% \\
% $
% \left\{T | (\forall \alpha_{1} \in T_1,  ((\alpha_{1}  \in T_2) \wedge (\alpha_{1}  \in T)) \right.$
% $ \left. \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \notin T_2)))\right.$
% \\
% $\left. \wedge(\forall \alpha_{2} \in T,(\alpha_{2} \in T_1)\vee(\alpha_{2} \in T_2))\right.$
% $ \left. \wedge (\forall \alpha_3 \in T,\ \xi_{\alpha_3}(T)=1)\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{6. EXCEPT: T1 except T2 \\ }
% $\left\{T_{1}, T_{2}\right\}\ EXCEPT $
% \\
% $
% \left\{T | (\forall \alpha_{1} \in T_1,  ((\alpha_{1}  \in T) \wedge (\alpha_{1}  \notin T_2) \right.$
% $ \left. \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \in T_2)))\right.$
% \\
% $\left. \wedge(\forall \alpha_{2} \in T,(\alpha_{2} \in T_1))\right.$
% $ \left. \wedge (\forall \alpha_3 \in T,\ \xi_{\alpha_3}(T)=1)\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{7. UNION ALL: T1 union all T2 \\ }
% $
% \left\{T_{1}, T_{2}\right\}\ UNION\ ALL $
% \\
% $\left\{T | (\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2,\right.$
% $\left. \alpha_{1} , \alpha_{2} \in T) \right.$
% \\
% $\left. \wedge(\forall \alpha_{3} \in T,(\alpha_{3} \in T_1)\vee(\alpha_{3} \in T_2))\right.$
% $ \left. \wedge (\forall \alpha_4 \in T,\ \xi_{\alpha_4}(T)=\xi_{\alpha_4}(T_1)+\xi_{\alpha_4}(T_2))\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{8. INTERSECT ALL: T1 intersect all T2 \\ }
% $\left\{T_{1}, T_{2}\right\}\ INTERSECT\ ALL $
% \\
% $
% \left\{T | (\forall \alpha_{1} \in T_1, \right.$
% $ \left.((\alpha_{1}  \in T_2) \wedge (\alpha_{1}  \in T) \right.$
% $ \left. \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \notin T_2)))\right\}$
% \\
% $ \left. \wedge (\forall \alpha_2 \in T,\ \right.$
% $\left. \xi_{\alpha_2}(T)=min(\xi_{\alpha_2}(T_1),\xi_{\alpha_2}(T_2)))\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{9. EXCEPT ALL: T1 except all T2 \\ }
% $\left\{T_{1}, T_{2}\right\}\ EXCEPT\ ALL $
% \\
% $
% \left\{T | (\forall \alpha_{1} \in T_1,\right. $
% $ \left.((\alpha_{1}  \in T) \wedge (\alpha_{1}  \notin T_2) \right.$
% $ \left. \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \in T_2)))\right\}$
% \\
% $ \left. \wedge (\forall \alpha_2 \in T,\ \right.$
% $ \left. \xi_{\alpha_2}(T)=max(\xi_{\alpha_2}(T_1)-\xi_{\alpha_2}(T_2)),0)\right\}
% $
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Aggregation operation}\\}
% \leftline{10. MIN: min($T.\beta$) \\ }
% $\left\{T,\beta\right\}\ MIN $
% \\
% $\left\{
% x_{min} | (x_{min} \in \pi_{\beta}(T),
% \right. $ 
% $\left. \Theta=(v \in \pi_{\beta}(T)\wedge(v < x_{min})),\ \sigma_{\Theta}(T)=\oslash \right\} $
% \\ \hspace*{\fill} \\
% \leftline{11. MAX: max($T.\beta$) \\ }
% $\left\{T,\beta\right\}\ MAX $
% \\
% $\left\{x_{max} | x_{max} \in \pi_{\beta}(T), \right. $
% $\left.\Theta=(v \in \pi_{\beta}(T) \wedge(v > x_{max})),\ \sigma_{\Theta}(T)=\oslash\right\}$
% \end{framed}
% \end{figure*}
% \begin{figure*}
% \begin{framed}
% \leftline{12. SUM: sum($T.\beta$) \\ }
% $\left\{T,\beta\right\}\ SUM\ \left\{x_{sum} | x_{sum}=\sum_{v \in \pi_{\beta}(T)}v,\right\}$
% \\ \hspace*{\fill} \\

% \leftline{13. COUNT: count($T.\beta$) \\ }
% $\left\{T,\beta\right\}\ COUNT\ \left\{x_{count} | x_{count}=\sum_{\alpha \in T}(\xi_{\alpha} (T))  \right\}$
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Group operation}\\}
% \leftline{14. GROUP BY: group by $T.\beta$\\ }
% $\left\{T,\beta\right\}\ GROUP BY $
% \\
% $\left\{T_{1}=(\overline{\beta},(\overline{\alpha_1},...,\overline{\alpha_k})) |\forall \overline{\alpha_i} \in\ (\overline{\alpha_1},...,\overline{\alpha_k}), \right.$
% $\left. (\forall\ v_{ij}\ \in\ \pi_{\beta}(\sigma_{TRUE}(\overline{\alpha_i})),(v_{ij}=v_{i1})   \right.$
% \\
% $\left. \wedge(\forall\ v_{xy}\ \in\ \pi_{\beta}(\sigma_{TRUE}(\overline{\alpha_x})),(v_{ij}\ne v_{xy}),(x\in(1,...,k))\wedge(x\ne i)))   \right.$
% \\
% $\left. \wedge(\forall \alpha_x \in T,\xi_{\alpha_x}(T_1)=\xi_{\alpha_x}(T))\right.$
% $\left. \wedge(\forall \alpha_y \in T_1,\xi_{\alpha_y}(T_1)=\xi_{\alpha_y}(T))\right\}$
% \\ \hspace*{\fill} \\
% \leftline{15. HAVING: having\ $\Theta$\\ }
% $\left\{T,\Theta\right\}\ HAVING $
% \\
% $\left\{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1)\\ \right.$
% $\left. \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)\right.$
% $\left. \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\right\}$
% \\ \hspace*{\fill} \\
% \leftline{16. DISTINCT: distinct\ $T.\beta$ \\ }
% $\left\{T,\beta\right\}\ DISTINCT $
% \\
% $\left\{T_{1} | (\forall \alpha \in T,\ \xi_{\alpha} (T_1)=1) \right.$
% $\left. \wedge(\forall \alpha_1 \in T_1,\ \alpha_1 \in T )\right\}$
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Condition}\\}
% \leftline{17. BETWEEN: between value1 and value2 \\ }
% $\left\{T,\beta,value_1,value_2\right\}\ BETWEEN $
% \\
% $\left\{\Theta |  \Theta=(v \in \pi_{\beta}(T), (v \ge value1) \wedge (v \le value2))\right\}$
% \\ \hspace*{\fill} \\
% \leftline{18. EXISTS:  exists($\Theta$) \\ }
% $\left\{\Theta \right\}\ EXISTS\ \left\{\Theta_1 | \Theta_1=(\Theta = TRUE)\right\}$
% \\ \hspace*{\fill} \\
% \leftline{19.  AND:  $\Theta_1$\ and\ $\Theta_2$ \\ }
% $\left\{\Theta_{1}, \Theta_{2}\right\}\ AND\ \left\{\Theta |  \Theta=\Theta_{1} \wedge \Theta_{2} \right\}$
% \\ \hspace*{\fill} \\
% \leftline{20. OR:  $\Theta_1$\ or\ $\Theta_2$ \\ }
% $\left\{\Theta_{1}, \Theta_{2}\right\}\ OR\ \left\{\Theta |  \Theta=\Theta_{1} \vee \Theta_{2} \right\}$
% \\ \hspace*{\fill} \\
% \leftline{21. NOT:  not $\Theta$ \\ }
% $\left\{\Theta_{1}\right\}\ NOT\ \left\{\Theta |  \Theta = \neg \Theta_{1}\right\}$
% \\ \hspace*{\fill} \\
% \leftline{22. t IS NULL:  t is null \\ }
% $\left\{t\right\}\ IS\ NULL\ \left\{\Theta |  \Theta = (t\ =\ NULL)\right\}$
% \\ \hspace*{\fill} \\
% \leftline{23. t IS NOT NULL:  t is not null \\ }
% $\left\{t\right\}\ IS\ NOT\ NULL\ \left\{\Theta |  \Theta = (t\ \ne\ NULL)\right\}$
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Join operation}\\}
% \leftline{24. NATURAL JOIN :  $T_1$ natural join $T_2$ \\ }
% $\left\{T_{1}, T_{2}\right\}\left\{NATURAL\ JOIN\right\}$
% \\
% $\left\{T | (\forall \beta_1 \in T_1.\overline{\beta},\beta_1 \in T.\overline{\beta},\xi_{\beta_1}(T)=1;\\ \right.$
% $\left. \forall \beta_2 \in T_2.\overline{\beta},\beta_2 \in T.\overline{\beta},\xi_{\beta_2}(T)=1;\right.)$
% \\
% $
% \left. \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1))\\ \right.$
% $
% \left. \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2)) \right\}$
% \end{framed}
% \end{figure*}






==> SemanticRules.tex <==
\begin{figure*}[tp]
\footnotesize
\begin{framed}
\leftline {\textbf{Query expression}\\}
\leftline{$1.\{\{T\}\}\ \text{FROM}\ \{\{T\}\}\ \ \ \ \ \ 2.\{\{T\}\}\ \text{SELECT}\ \widehat{\beta}\ \{\{\pi_{\widehat{\beta}}(T)\}\}$}
\leftline{$3.\{\{T\}\}\ 
\text{WHERE}\ \Theta
\ \{\{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_{1}) 
\wedge(\forall \alpha \notin \sigma_{\Theta} (T),\alpha \notin T_{1})
\wedge(\forall \alpha \in T_1, \xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}\}$}
% \leftline {2. SELECT: select\ $T.\overline{\beta}$\\}
% $$
% \frac{\{T,\overline{\beta}\}}{\{T_1|T_1=\{\pi_{\overline{\beta}}(T)\}\}}
% $$
% $
% \{T,\Theta\}
% WHERE
% \{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_{1}) 
% \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_{1})
% \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}
% $
\leftline {\textbf{Join operation}\\}
% $$
% \{T_{1}, T_{2}\}
% NATURAL\ JOIN \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
% \{T_{1}, T_{2}\}
% LEFT\ JOIN \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
% \{T_{1}, T_{2}\}
% RIGHT\ JOIN \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  
% \{T_{1}, T_{2}\}
% FULL\ JOIN 
% $$
% $$
% \begin{aligned}
%     \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta}) 
%     \wedge(\beta \in T_2.\overline{\beta})) \ \ \ \ \ \ \ \ \ 
%     \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee((\beta \in T_1.\overline{\beta}) 
%     \ \ \ \ \ \ \ \ \ \ 
%     \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_2.\overline{\beta})\vee((\beta \in T_1.\overline{\beta})
%     \ \ \ \ \ \ \ \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee(
%     \beta \in T_2.\overline{\beta}))
%  \wedge\\ 
%  \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),
%  \ \ \ \ \ \ \ \ \ \ \wedge(\beta \in T_2.\overline{\beta})))\wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),
%  \ \ \ \ \ \ \ \ \ \ \wedge(\beta \in T_2.\overline{\beta})))
%  \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),
%  \ \ \ \ \ \ \ \ (\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\\
% \xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1)) 
% \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),
% \ \ \ \ \ \ \ \ \ \ \ \xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1)) 
% \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),
% \ \ \ \ \ \ \ \ \ \ \ \ \xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1)) 
% \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\ \ \ \ \ \ \ \ \xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))
% \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),
% \\
% \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
% \ \ \ \ \ \ \ \ \ \ \ \
% \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
% \ \ \ \ \ \ \ \ \ \ \ \ \ 
% \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
% \ \ \ \ \ \ \ \ \ \ 
% \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
% \end{aligned}
% $$
% $$
% \{T,\Theta\}
% ON
% \begin{aligned}
%     \{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1) 
%  \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)
%  \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}
% \end{aligned}
% $$
\leftline{
$4.
\{\{T_{1}, T_{2}\}\}\ 
\text{NaturalJoin}\ 
\begin{aligned}
    \{\{T | 
    % (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta}))
    &((\forall \alpha \in \pi_{T_1.{\overline{\beta}}}(T),\alpha \in T_1)\wedge(\forall \alpha \in \pi_{T_2.{\overline{\beta}}}(T),\alpha \in T_2))
    \wedge(\forall \alpha_1 \in T_1,\alpha_2 \in T_2,\\
    &(\forall \beta \in \overline{\beta}_I, \text{iff} (\beta \in T_1.\overline{\beta})\wedge (\beta \in T_2.\overline{\beta}),
    \pi_{\overline{\beta}_I}(\{\alpha_1\}) = \pi_{\overline{\beta}_I}(\{\alpha_2\}))
    \wedge(\alpha_1 \circ \alpha_2 \in T))\}\}
 % \forall \alpha \in \pi_{T.{\overline{\beta}}}(T),(\alpha \in \pi_{T_1.{\overline{\beta}}}(T_1))\wedge(\alpha \in \pi_{T_2.{\overline{\beta}}}(T_2)) \wedge(\xi_{\alpha}(T)=1)\} 
% &\wedge(\forall \alpha_2 \in \pi_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \pi_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
$}
~\\
~\\
\leftline{
$5.
\{\{T_{1}, T_{2}\}\}\ 
\text{LeftJoin}\ 
\begin{aligned}
    \{\{T | 
    % (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee((\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta})))
    &\forall \beta \in \overline{\beta}_I, \text{iff} (\beta \in T_1.\overline{\beta})\wedge (\beta \in T_2.\overline{\beta}), (\forall \alpha \in T, ((\pi_{\overline{\beta}_I}(\{\alpha\}) \in T_2) \wedge ((\pi_{T_1.\overline{\beta}}({\alpha}) \in T_1)\wedge(\pi_{T_2.\overline{\beta}}({\alpha}) \in T_2))) \vee\\
    &((\pi_{\overline{\beta}_I}(\{\alpha\}) \notin T_2) \wedge ((\pi_{T_1.\overline{\beta}}(\{\alpha\}) \in T_1)\wedge(\pi_{T.\overline{\beta}-T_1.\overline{\beta}}(\{\alpha\}) = [null,...,null]_{|T.\overline{\beta}|-|T_1.\overline{\beta}|}))))\wedge\\
    &(\forall \alpha_1 \in T_1),((\exists \alpha_2 \in T_2),(\pi_{\overline{\beta}_I}(\{\alpha_1\}) = \pi_{\overline{\beta}_I}(\{\alpha_2\}))\wedge(\alpha_1 \circ \alpha_2 \in T)) \vee\\
    &((\nexists \alpha_2 \in T_2),(\pi_{\overline{\beta}_I}(\{\alpha_1\}) = \pi_{\overline{\beta}_I}(\{\alpha_2\}))\wedge(\alpha_1 \circ [null,...,null]_{|T.\overline{\beta}|-|T_1.\overline{\beta}|} \in T))
%  (\forall \alpha \in \pi_{T_1.{\overline{\beta}}}(T),\alpha \in \pi_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha}(T)=1) 
% \wedge(\forall \alpha \in \pi_{T_2.{\overline{\beta}}}(T),\alpha \in \pi_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha}(T)=1)
\}\}
\end{aligned}
$}
% \leftline{
% $6.
% \{T_{1}, T_{2}\}
% \text{RightJoin}
% \begin{aligned}
%     \{T | 
%     % (\forall \beta \in T.\overline{\beta},(\beta \in T_2.\overline{\beta})\vee((\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta})))
%  (\forall \alpha \in \pi_{T_1.{\overline{\beta}}}(T),\alpha \in \pi_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha}(T)=1) 
% \wedge(\forall \alpha \in \pi_{T_2.{\overline{\beta}}}(T),\alpha \in \pi_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha}(T)=1) \}
% \end{aligned}
% $}
% \leftline{
% $7.
% \{T_{1}, T_{2}\}
% \text{FullJoin}
% \begin{aligned}
%     \{T | 
%     % (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee(\beta \in T_2.\overline{\beta}))
%  (\forall \alpha \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha}(T)=1)
% \wedge(\forall \alpha \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha}(T)=1) \}
% \end{aligned}
 % $}
\leftline{
$6.
\{\{T\}\}\ 
\text{ON}\ \Theta\ 
\begin{aligned}
    \{\{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_{1}) 
\wedge(\forall \alpha \notin \sigma_{\Theta} (T),\alpha \notin T_{1})
\wedge(\forall \alpha \in T_1, \xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}\}
\end{aligned}
$}
\leftline {\textbf{Logical operation}\\}
\leftline{
$7.
\text{EXISTS}\ \Theta\ 
\begin{aligned}
    \{\{\Theta == TRUE\}\}
\end{aligned}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
$
$8.
% \{\Theta\}\
\Theta\ \text{IS\ NULL}\ 
\begin{aligned}
    \{\{\Theta\ ==\ NULL\}\}
\end{aligned}
$}
% \leftline{19.  AND:  $\Theta_1$\ and\ $\Theta_2$ \\ }
% $$\frac{
% \{\Theta_{1}, \Theta_{2}\}
% }{
% \begin{aligned}
%     \{\Theta |  \Theta=\Theta_{1} \wedge \Theta_{2} \}
% \end{aligned}
% }$$
\leftline {\textbf{Aggregation operation(AGG)}\\}
\leftline{
$9.
\{\{T\}\}\ 
\text{MIN}\ \beta\ 
\begin{aligned}
    \{\{
v_{min} \ s.t.\  v_{min} \in \pi_{\beta}(T) \wedge(\forall v \in \pi_{\beta}(T), \sigma_{(v < v_{min})}(\pi_{\beta}(T))=\oslash) \}\}
\end{aligned}\ \ \ \ \ \ \ 10.
\{\{T\}\}\ 
\text{SUM}\ \beta\ 
\begin{aligned}
    \{\{\sum_{v \in \pi_{\beta}(T)}v\}\}
\end{aligned}
$}
\leftline{
$ 11.
\{\{T\}\}\ 
\text{MAX}\ \beta\ 
\begin{aligned}
    \{\{
v_{max} \ s.t.\  v_{max} \in \pi_{\beta}(T) \wedge(\forall v \in \pi_{\beta}(T), \sigma_{(v > v_{max})}(\pi_{\beta}(T))=\oslash) \}\}
\end{aligned}\ \ \ \ \ \ \ 12.
\{\{T\}\}\ 
\text{COUNT}\ \widehat{\beta}\ 
\begin{aligned}
    \{\{\sum_{\alpha \in \pi_{\widehat{\beta}}(T)}(\xi_{\alpha} (T)) \}\}
\end{aligned}
$}

% \leftline{13. COUNT: count($T.\beta$) \\ }
% $$\frac{
% \{T,\beta\}
% }{
% \begin{aligned}
%     \{x_{count} | x_{count}=\sum_{\alpha \in T}(\xi_{\alpha} (T)) \}
% \end{aligned}
% }$$
% \leftline{21. NOT:  not $\Theta$ \\ }
% $$\frac{
% \{\Theta_{1}\}
% }{
% \begin{aligned}
%     \{\Theta |  \Theta = \neg \Theta_{1}\}
% \end{aligned}
% }$$
% \leftline{23. $\Theta$ IS NOT NULL:  $\Theta$ is not null \\ }
% $$\frac{
% \{\Theta\}\
% }{
% \begin{aligned}
%     \{\Theta_1 |  \Theta_1 = (\Theta\ \ne\ NULL)\}
% \end{aligned}
% }$$
\leftline {\textbf{Group operation}\\}
\leftline{
$13.
\{\{T\}\}\ 
\text{GroupBy}\ \beta\ 
\begin{aligned}
    \{\{&T_{1}=((\widehat{\alpha_1},...,\widehat{\alpha_k})) |\forall \widehat{\alpha_p} \in\ (\widehat{\alpha_1},...,\widehat{\alpha_k}), 
 (\forall\ v_{ij}\ \in\ \pi_{\beta}(\widehat{\alpha_p}),(v_{ij}=v_{i1})   
 \wedge(\forall\ v_{xy}\ \in \pi_{\beta}(\widehat{\alpha_q}),(q\in(1,...,k))\wedge(q\ne p),\\ 
&(v_{ij}\ne v_{xy})
))   
 \wedge(\forall \alpha_q \in T,\xi_{\alpha_q}(T_1)=\xi_{\alpha_q}(T))
\wedge(\forall \alpha_r \in T_1,\xi_{\alpha_r}(T_1)=\xi_{\alpha_r}(T))\}\}
\end{aligned}
$}
\leftline{
$14.
\{\{T\}\}\ 
\text{HAVING}\ \Theta\ 
\begin{aligned}
    \{\{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_{1}) 
\wedge(\forall \alpha \notin \sigma_{\Theta} (T),\alpha \notin T_{1})
\wedge(\forall \alpha \in T_1, \xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}\}
\end{aligned}
% \{T,\beta\}\
% ORDER\ BY
% \begin{aligned}
%     \{T_{1} | (\forall \alpha \in T_1,\ \xi_{\alpha} (T_1)=\xi_{\alpha} (T)) 
% \end{aligned}
$}
~\\
\leftline{
$15.
\{\{T\}\}\ 
\text{DISTINCT}\ 
\begin{aligned}
    \{\{T_{1} | (\forall \alpha \in T,\ \xi_{\alpha} (T_1)=1) 
 \wedge(\forall \alpha \in T_1,\ \alpha \in T )\}\}
\end{aligned}
% \begin{aligned}
% \wedge(\forall \alpha \in T,\ \xi_{\alpha} (T)=\xi_{\alpha} (T_1))\wedge(\forall \alpha_i \in \sigma_{T_1.{\overline{\beta}}}(T_1),\ \alpha_i > \alpha_{i+1} )\}
% \end{aligned}
$}
~\\
\leftline{
$16.
\{\{T\}\}\ 
\text{OrderBy}\ \beta\ 
\begin{aligned}
    \{\{T_{1} | (\forall \alpha \in T_1,\ \xi_{\alpha} (T_1)=\xi_{\alpha} (T)) 
\wedge(\forall \alpha \in T,\ \xi_{\alpha} (T)=\xi_{\alpha} (T_1))
 \wedge(\forall v_i, v_j\in \sigma_{T_1.{\beta}}(T_1), i<j \text{\space} \text{iff} \ v_i > v_{j} )\}\}
\end{aligned}
$}
% $$
% \{T,\beta\}\
% ORDER\ BY\ ASC
% \begin{aligned}
%     \{T_{1} | (\forall \alpha \in T_1,\ \xi_{\alpha} (T_1)=\xi_{\alpha} (T)) 
% \wedge(\forall \alpha \in T,\ \xi_{\alpha} (T)=\xi_{\alpha} (T_1))
%  \wedge(\forall \alpha_i \in \sigma_{T_1.{\overline{\beta}}}(T_1),\ \alpha_i < \alpha_{i+1} )\}
% \end{aligned}
% $$
\leftline {\textbf{Collection operation}}
\leftline{$17.
    \{\{T_{1}, T_{2}|T_1.\overline{\beta} = T_2.\overline{\beta}\}\}\ \text{UNION}\ 
\begin{aligned}
    \{\{T | (\forall \alpha \in T, (\xi_{\alpha}(T)=1)\wedge((\alpha \in T_1)\vee(\alpha \in T_2)))\wedge(\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2,  
 \alpha_{1} , \alpha_{2} \in T) \}\}
\end{aligned}
$}
\leftline{
$18.\{\{T_{1}, T_{2}|T_1.\overline{\beta} = T_2.\overline{\beta}\}\}\ \text{INTERSECT}\ 
\begin{aligned}
    \{\{&T | (\forall \alpha \in T, (\xi_{\alpha}(T)=1)\wedge((\alpha \in T_1)\wedge(\alpha \in T_2)))\wedge(\forall \alpha \in T_1,
 ((\alpha  \in T_2) \wedge (\alpha  \in T)) \\
 &\vee ((\alpha  \notin  T) \wedge (\alpha  \notin T_2)))
 \wedge(\forall \alpha \in T_2,
 ((\alpha  \in T_1) \wedge (\alpha  \in T)) 
 \vee ((\alpha  \notin  T) \wedge (\alpha  \notin T_1)))\}\}
\end{aligned}
 $}
 ~\\
 \leftline{
$19.
\{\{T_{1}, T_{2}|T_1.\overline{\beta} = T_2.\overline{\beta}\}\}\  \text{EXCEPT}\ 
\begin{aligned}
    \{\{&T | (\forall \alpha \in T,(\alpha \in T_1) \wedge (\xi_{\alpha}(T)=1)\wedge (\xi_{\alpha}(T_1)>\xi_{\alpha}(T_2)))\\
    &\wedge(\forall \alpha \in T_1, ((\alpha  \in T) \wedge (\xi_{\alpha}(T_1)>\xi_{\alpha}(T_2)) 
 \vee ((\alpha  \notin T) \wedge (\xi_{\alpha}(T_1)\leq\xi_{\alpha}(T_2))))\}\}
\end{aligned}
$}
~\\
\leftline{
$20.
    \{\{T_{1}, T_{2}|T_1.\overline{\beta} = T_2.\overline{\beta}\}\}\ \text{UnionAll}\ 
\begin{aligned}
    \{\{&T | (\forall \alpha \in T,
\alpha \in T_1
\vee \alpha \in T_2)
 \wedge (\forall \alpha \in T,
 \xi_{\alpha}(T)=\xi_{\alpha}(T_1)+\xi_{\alpha}(T_2))\\
 &\wedge(\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2,
 \alpha_{1} , \alpha_{2} \in T) 
 \}
\end{aligned}
$}
% ~\\
% \leftline{
% $23.
% \{\{T_{1}, T_{2}|T_1.\overline{\beta} = T_2.\overline{\beta}\}\}\ \text{IntersectAll}\ 
% \begin{aligned}
%     \{\{&T | (\forall \alpha \in T, (\xi_{\alpha}(T)=min(\xi_{\alpha}(T_1),\xi_{\alpha}(T_2)))\wedge(\alpha \in T_1 \wedge \alpha \in T_2))\wedge(\forall \alpha \in T_1,
%  (\alpha  \in T_2 \wedge \alpha  \in )) \\
%  &\vee (\alpha  \notin  T \wedge \alpha  \notin T_2))
%  \wedge(\forall \alpha \in T_2,
%  (\alpha  \in T_1 \wedge \alpha  \in T) 
%  \vee (\alpha  \notin  T \wedge \alpha  \notin T_1))\}\}
% \end{aligned}
% % \begin{aligned}
% %     \{&T | (\forall \alpha \in T_1, 
% % ((\alpha  \in T_2) \wedge (\alpha  \in T) 
% % \vee ((\alpha  \notin T)
% % \wedge (\alpha  \notin T_2))))
% % \wedge(\forall \alpha \in T_2, 
% % ((\alpha  \in T_1) \wedge (\alpha  \in T) 
% % \vee \\ 
% % &((\alpha  \notin T)
% % \wedge (\alpha  \notin T_1)))) 
% %  \wedge (\forall \alpha \in T,\ 
% % \xi_{\alpha}(T)=min(\xi_{\alpha}(T_1),\xi_{\alpha}(T_2)))\}
% % \end{aligned}
% $}
% ~\\
% \leftline{
% $24.
% \{\{T_{1}, T_{2}|T_1.\overline{\beta} = T_2.\overline{\beta}\}\}\ \text{ExceptAll}\ 
% \begin{aligned}
%     \{\{&T | (\forall \alpha \in T,(\alpha \in T_1) \wedge (\xi_{\alpha}(T)=\xi_{\alpha}(T_1)-\xi_{\alpha}(T_2))\wedge (\xi_{\alpha}(T_1)>\xi_{\alpha}(T_2)))\\
%     &\wedge(\forall \alpha \in T_1, ((\alpha  \in T) \wedge (\xi_{\alpha}(T_1)>\xi_{\alpha}(T_2)) 
%  \vee ((\alpha  \notin T) \wedge (\xi_{\alpha}(T_1)\leq \xi_{\alpha}(T_2))))\}\}
% \end{aligned}
% % \begin{aligned}
% %     \{T | (\forall \alpha \in T_1,
% % ((\alpha  \in T) \wedge (\alpha  \notin T_2) 
% %  \vee ((\alpha  \notin T) \wedge  (\alpha  \in T_2)))\}
% %  \wedge (\forall \alpha \in T,
% %  \xi_{\alpha}(T)=max(\xi_{\alpha}(T_1)-\xi_{\alpha}(T_2),0))\}
% % \end{aligned}
% $}
\leftline {\textbf{Function operation}\\}
\leftline{
$21.
% \{str,length,str1\}
\text{RPAD}(str,l,str1)\ 
\begin{aligned}
    \{\{str2 \ s.t.\  (|str2|=l)
\wedge(str2[0,|str|]=str)
 \wedge
 (\forall i \in (|str|,|str2|+1),
str2[i]=str1[(i-|str|)\%(|str1|)]) \}\}
\end{aligned}
$}
% \leftline{
% $2.
% \{str,length,str1\}
% \text{LPAD}
% \begin{aligned}
%     \{&str2 | (|str2|=length) 
%  \wedge(str2[|str2|-|str|,|str2|]\\
%  &=str) 
% \wedge(\forall i \in (0,|str2|-|str|),
% str2[i]=str1[i\%|str1|]) \}
% \end{aligned}
% $}
% \leftline{
% $3.
% \{str,length\}
% \text{LEFT}
% \begin{aligned}
%     \{str1 | str1=str[0,length]\}
% \end{aligned}
% \ \ \ \ \ \ \ 4.
% \{str,length\}
% \text{RIGHT}
% \begin{aligned}
%     \{str1 | str1=str[|str|-length,|str|] \}
% \end{aligned}
% $}
% \leftline{
% $5.
% \{str1,str2\}
% \text{INSTR}
% \begin{aligned}
%     \{n | str2=str1[n,n+|str2|]
%  \wedge(\forall i \in (0,n-1),str1[i,i+|str2|]\ne str2\}
% \end{aligned}
% $}
% \leftline{locate/position($str1,str2,start$) \\}
~\\
\leftline{
$22.
% \{str1,str2,start\}
\text{LOCATE/POSITION}(str1,str2,index)\ 
\begin{aligned}
    \{\{v \ s.t.\  str1=str2[v,v+|str1|]
\wedge(\forall i \in (index,v),str2[i:i+|str1|]\ne str1\}\}
\end{aligned}
$}
% \leftline{substr/substring/mid($str,start,length$) \\ }
% \leftline{substring_index($str,char,index$) \\ }
~\\
% \leftline{
% $4.
% \{str,char,index\}
% \text{SUBSTRING\_INDEX}
% \begin{aligned}
%     \{str1 | (str1=str[0,|str1|])
%  \wedge(str[|str1|]=index)
% \wedge(\xi_{char}(str1)=index-1)\}
% \end{aligned}
% $}
\leftline{
$23.
% \{str,\overline{str}\}
\text{FIND\_IN\_SET/FIELD}(str,STR)\ 
\begin{aligned}
    \{\{v \ s.t.\  (STR[v]=str) 
\wedge(\forall i \in (0,v),STR[i] \ne str)\}\}
\end{aligned}
$}
~\\
% \leftline{
% $6.
% \{index,\overline{str}\}
% \text{ELT}
% \begin{aligned}
%     \{str | (\overline{str}[index]=str)
% \wedge(\forall i \in (0,index),\overline{str}[i]\ne str)\}
% \end{aligned}
% $}
\leftline{
$24. 
% \{\Theta,\Theta_{1},\Theta_{2}\}
% \text{CASE/IF}
\begin{aligned}
    \frac { \{\Theta \wedge P\}\ \Theta_{1}\ \{Q\}\ ,\ \{\neg \Theta \wedge P \}\ \Theta_{2}\ \{Q\} }
              { \{P\}\ \textbf{if}\ \Theta\ \textbf{then}\ \Theta_{1}\ \textbf{else}\ \Theta_{2}\ \textbf{endif}\ \{Q\} }
    % \{\Theta = TRUE\}
\end{aligned}
$}
% $$
% \{\Theta,\Theta_{1},\Theta_{2}\}
% CASE/IF
% \begin{aligned}
%     \{\Theta_{3} | \Theta_{3}=\Theta_{1}, \Theta=TRUE;
% \Theta_{3}=\Theta_{2}, \Theta=FALSE\}
% \end{aligned}
% $$
~\\
% \leftline{
% $8.
% \{\Theta_{1},\Theta_{2}\}
% \text{NULLIF}
% \begin{aligned}
%     \{\Theta_{1}=\Theta_{2}\}
% \end{aligned}
% $}
% ~\\
% \leftline{
% $9.
% \{\overline{str}\}
% \text{COALESCE}
% \begin{aligned}
%     \{v | (\overline{str}[v]=NULL) 
% \wedge(\forall i \in (0,v),\overline{str}\ne NULL)\}
% \end{aligned}
% $}
\leftline {\textbf{Compound semantics}\\}
\leftline{25. CQ1: SELECT $\beta$ FROM T\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 26. CQ2: SELECT $\beta$ FROM $T_1$ Join operation $T_2$
% \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 3. $T_1,T_2$ Collection Operation $T$
\\ }
$\frac{\left\{\left\{T\right\}\right\}\ \text{FROM}\ \left\{\left\{T\right\}\right\},\ \left\{\left\{T\right\}\right\}\ \text{SELECT}\ \beta\  \{\{\pi_{\beta}(T)\}\}}{\left\{\left\{T\right\}\right\}\ \text{FROM;\ SELECT}\ \beta \{\{\pi_{\beta}(T)\}\}}\ \ \ \ \frac{\{\left\{T_1,T_2\right\}\}\ \text{JOIN\ operation}\ \left\{\left\{T\right\}\right\},\left\{\left\{T\right\}\right\}\ \text{FROM}\ \left\{\left\{T\right\}\right\},\ \left\{\left\{T\right\}\right\}\ \text{SELECT}\ \beta\  \{\{\pi_{\beta}(T)\}\}}{\{\left\{T_1,T_2\right\}\}\ \text{Join\ operation;\ FROM;\ SELECT}\ \beta\  \{\{\pi_{\beta}(T)\}\}}   
    % \ \ \ \ \{T_1,T_2\}\ \text{Collection\ Operation}\ \{T\}
    $
~\\
~\\
\leftline{27. CQ3: SELECT $\beta$ FROM T WHERE $\Theta$\\}
$
\frac{\left\{\left\{T\right\}\right\}\ \text{FROM}\ \left\{\left\{T\right\}\right\},\ \left\{\left\{T\right\}\right\}\ \text{WHERE}\ \Theta\  \{\left\{\sigma_{\Theta}(T)\right\}\},\{\left\{\sigma_{\Theta}(T)\right\}\}\ \text{SELECT}\ \beta\   \{\{\pi_{\beta}(\sigma_{\Theta}(T))\}\}}{\left\{\left\{T\right\}\right\}\ \text{FROM;\ WHERE}\ \Theta;\ \text{SELECT}\ \beta\    \{\{\pi_{\beta}(\sigma_{\Theta}(T))\}\}}$
~\\
~\\
\leftline{28. CQ4: SELECT AGG ($\beta$) FROM T\\}
$
\frac{\left\{\left\{T\right\}\right\}\ \text{FROM}\ \left\{\left\{T\right\}\right\},\ \left\{\left\{T\right\}\right\}\ \text{AGG}\ \beta\ \{\left\{x\right\}\},\left\{\left\{T\right\}\right\}\ \text{SELECT}\ x\ \{\{\pi_{x}(T)\}\}}{\left\{\left\{T\right\}\right\}\ \text{FROM;AGG $\beta$;\ SELECT}\   \{\{\pi_{x}(T)\}\}}$
% ~\\
% ~\\
% \leftline{4. CQ4: SELECT AGG ($\beta$) FROM T\\}
% $\frac{\left\{\left\{T\right\}\right\}\ \text{FROM}\ \left\{\left\{T\right\}\right\},\ \left\{\left\{T\right\}\right\}\ \text{AGG}\ \beta\ \left\{x\right\},\left\{\left\{T\right\}\right\}\ \text{SELECT}\ x\ \{\pi_{x}(T)\}}{\left\{\left\{T\right\}\right\}\ \text{FROM;AGG $\beta$;\ SELECT}  \{\pi_{x}(T)\}}$
~\\
~\\
\leftline{29. CQ5: SELECT $\beta$ FROM T GROUP BY $\beta$ HAVING $\Theta$ \\ }
$\frac{\left\{\left\{T\right\}\right\}\ \text{FROM}\ \left\{\left\{T\right\}\right\},\ \left\{\left\{T\right\}\right\}\ \text{GroupBy}\ \beta\ \{\left\{T_1\right\}\},\ \{\left\{T_1\right\}\}\ \text{HAVING}\ \Theta\  \{\left\{\sigma_{\Theta}(T_1)\right\}\},\{\left\{\sigma_{\Theta}(T_1)\right\}\}\ \text{SELECT}\ \beta\   \{\{\pi_{\beta}(\sigma_{\Theta}(T_1))\}\}}{\left\{\left\{T\right\}\right\}\ \text{FROM;\ GroupBy\ $\beta$;\ HAVING}\ \Theta;\ \text{SELECT}\ \beta\    \{\{\pi_{\beta}(\sigma_{\Theta}(T_1))\}\}}$
% \\ \hspace*{\fill} \\
% $\frac{\left\{T_2,\beta_1\right\}\ ORDER\ BY \left\{T_3\right\} }{\left\{T_2,\beta_1\right\}\ ORDER\ BY;\     \left\{T_3\right\}}$
\\ \hspace*{\fill} \\
\leftline{30. CQ6: SELECT $\beta$ FROM T ORDER BY $\beta$ ASC/DESC\\ } 
$\frac{\left\{\left\{T\right\}\right\}\ \text{FROM}\ \left\{\left\{T\right\}\right\},\ \left\{\left\{T\right\}\right\}\ \text{SELECT}\ \beta \{\{\pi_{\beta}(T)\}\},\{\{\pi_{\beta}(T)\}\}\ \text{OrderBy} \beta\ \{\left\{T_1\right\}\} \ }{\left\{\left\{T\right\}\right\}\ \text{FROM;\ SELECT $\beta$;\ OrderBy $\beta$;}\ \{\left\{T_1\right\}\} }$\ \ 
\\ \hspace*{\fill} \\
\leftline{31. CQ7: CQi Collection operation CQj\\ } 
$\frac{\{\left\{T_i\right\}\}\ \text{CQi}\ \{\{T_1\}\},\{\left\{T_j\right\}\}\ \text{CQj}\ \{\{T_2\}\},\{\{T_1,T_2\}\}\ \text{Collection Operation}\ \{\{T\}\}}{\{\left\{T_1,T_2\right\}\}\ \text{CQi;\ CQj;\ Collection Operation;}\ \left\{\left\{T\right\}\right\} }$ 
\end{framed}
\caption{Selected Semantic rules for SQL}
\label{fig:semantic1}
\end{figure*}

==> formal_semantic.tex <==
\begin{figure*}
{\footnotesize
\begin{framed}
\leftline {\textbf{Query expression}\\}
\leftline{$1.\{T\}\text{FROM}\{T\}\ \ \ \ 2.\{T,\overline{\beta}\}\text{SELECT}\{\pi_{\overline{\beta}}(T)\}\ \ \ 3.\{T,\Theta\}
\text{WHERE}
\{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_{1}) 
\wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_{1})
\wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}$}
% \leftline {2. SELECT: select\ $T.\overline{\beta}$\\}
% $$
% \frac{\{T,\overline{\beta}\}}{\{T_1|T_1=\{\pi_{\overline{\beta}}(T)\}\}}
% $$
% $
% \{T,\Theta\}
% WHERE
% \{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_{1}) 
% \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_{1})
% \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}
% $
\leftline {\textbf{Collection operation}}
\leftline{$4.
    \left\{T_{1}, T_{2}\right\}\text{UNION}
\begin{aligned}
    \{T | (\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2,  
 \alpha_{1} , \alpha_{2} \in T) \wedge(\forall \alpha_{3} \in T, 
(\alpha_{3} \in T_1)\vee(\alpha_{3} \in T_2))
 \wedge (\forall \alpha_4 \in T,\ \xi_{\alpha_4}(T)=1)\}
\end{aligned}
$}
\leftline{5.
$\{T_{1}, T_{2}\}\ \text{INTERSECT}
\begin{aligned}
    \{&T | (\forall \alpha_{1} \in T_1,
 ((\alpha_{1}  \in T_2) \wedge (\alpha_{1}  \in T)) 
 \vee ((\alpha_{1}  \notin  T) \wedge (\alpha_{1}  \notin T_2)))\\
 &\wedge(\forall \alpha_{2} \in T,
(\alpha_{2} \in  T_1)\vee(\alpha_{2} \in T_2))
 \wedge (\forall \alpha_3 \in T,\ \xi_{\alpha_3}(T)=1)\}
\end{aligned}
 $}
 \leftline{6.
$
\{T_{1}, T_{2}\} \text{EXCEPT}
\begin{aligned}
    \{T | (\forall \alpha_{1} \in T_1, 
 ((\alpha_{1}  \in T) \wedge (\alpha_{1}  \notin T_2) 
 \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \in T_2)))\wedge(\forall \alpha_{2} \in T,(\alpha_{2} \in T_1))
 \wedge (\forall \alpha_3 \in T,\ \xi_{\alpha_3}(T)=1)\}
\end{aligned}
$}
\leftline{7.
$
    \{T_{1}, T_{2}\}\text{UnionAll}
\begin{aligned}
    \{T | (\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2,
 \alpha_{1} , \alpha_{2} \in T) 
 \wedge(\forall \alpha_{3} \in T,
(\alpha_{3} \in T_1)
\vee(\alpha_{3} \in T_2))
 \wedge (\forall \alpha_4 \in T,
 \xi_{\alpha_4}(T)=\xi_{\alpha_4}(T_1)+\xi_{\alpha_4}(T_2))\}
\end{aligned}
$}
\leftline{8.
$
\{T_{1}, T_{2}\}\text{IntersectAll}
\begin{aligned}
    \{T | (\forall \alpha_{1} \in T_1, 
((\alpha_{1}  \in T_2) \wedge (\alpha_{1}  \in T) 
\vee ((\alpha_{1}  \notin T)
\wedge (\alpha_{1}  \notin T_2)))\}
 \wedge (\forall \alpha_2 \in T,\ 
\xi_{\alpha_2}(T)=min(\xi_{\alpha_2}(T_1),\xi_{\alpha_2}(T_2)))\}
\end{aligned}
$}
\leftline{9.
$
\{T_{1}, T_{2}\}\text{ExceptAll} 
\begin{aligned}
    \{T | (\forall \alpha_{1} \in T_1,
((\alpha_{1}  \in T) \wedge (\alpha_{1}  \notin T_2) 
 \vee ((\alpha_{1}  \notin T) \wedge  (\alpha_{1}  \in T_2)))\}
 \wedge (\forall \alpha_2 \in T,
 \xi_{\alpha_2}(T)=max(\xi_{\alpha_2}(T_1)-\xi_{\alpha_2}(T_2)),0)\}
\end{aligned}
$}
\leftline {\textbf{Aggregation operation}\\}
\leftline{10.
$
\{T,\beta\}
\text{MIN}
\begin{aligned}
    \{
x_{min} | (x_{min} \in \pi_{\beta}(T),
 \Theta=(v \in \pi_{\beta}(T)\wedge(v < x_{min})),\ \sigma_{\Theta}(T)=\oslash \}
\end{aligned}\ \ \ \ \ \ \ 12.
\{T,\beta\}\
\text{SUM}
\begin{aligned}
    \{x_{sum} | x_{sum}=\sum_{v \in \pi_{\beta}(T)}v\}
\end{aligned}
$}
\leftline{
$ 11.
\{T,\beta\}
\text{MAX}
\begin{aligned}
    \{x_{max} | (x_{max} \in  \pi_{\beta}(T), 
\Theta=(v \in \pi_{\beta}(T) \wedge(v > x_{max})),\ \sigma_{\Theta}(T)=\oslash\}
\end{aligned}\ \ \ \ \ \ \ 13.
\{T,\beta\}
\text{COUNT}
\begin{aligned}
    \{x_{count} | x_{count}=\sum_{\alpha \in T}(\xi_{\alpha} (T)) \}
\end{aligned}
$}

% \leftline{13. COUNT: count($T.\beta$) \\ }
% $$\frac{
% \{T,\beta\}
% }{
% \begin{aligned}
%     \{x_{count} | x_{count}=\sum_{\alpha \in T}(\xi_{\alpha} (T)) \}
% \end{aligned}
% }$$
\leftline {\textbf{Group operation}\\}
\leftline{
$14.
\{T,\beta\}\
\text{GroupBy}
\begin{aligned}
    \{T_{1}=(\overline{\beta},(\overline{\alpha_1},...,\overline{\alpha_k})) |\forall \overline{\alpha_i} \in\ (\overline{\alpha_1},...,\overline{\alpha_k}), 
 (\forall\ v_{ij}\ \in\ \pi_{\beta}(\overline{\alpha_i}),(v_{ij}=v_{i1})   
 \wedge(\forall\ v_{xy}\ \in \pi_{\beta}(\overline{\alpha_x}), 
(v_{ij}\ne v_{xy}),\\
(x\in(1,...,k))\wedge(x\ne i)))   
 \wedge(\forall \alpha_x \in T,\xi_{\alpha_x}(T_1)=\xi_{\alpha_x}(T))
\wedge(\forall \alpha_y \in T_1,\xi_{\alpha_y}(T_1)=\xi_{\alpha_y}(T))\}
\end{aligned}
$}
\leftline{
$15.
\{T,\Theta\}
\text{HAVING}
\begin{aligned}
    \{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1) 
 \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)
 \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}
\end{aligned}
% \{T,\beta\}\
% ORDER\ BY
% \begin{aligned}
%     \{T_{1} | (\forall \alpha \in T_1,\ \xi_{\alpha} (T_1)=\xi_{\alpha} (T)) 
% \end{aligned}
$}
\leftline{
$16.
\{T,\beta\}\
\text{DISTINCT}
\begin{aligned}
    \{T_{1} | (\forall \alpha \in T,\ \xi_{\alpha} (T_1)=1) 
 \wedge(\forall \alpha_1 \in T_1,\ \alpha_1 \in T )\}
\end{aligned}
% \begin{aligned}
% \wedge(\forall \alpha \in T,\ \xi_{\alpha} (T)=\xi_{\alpha} (T_1))\wedge(\forall \alpha_i \in \sigma_{T_1.{\overline{\beta}}}(T_1),\ \alpha_i > \alpha_{i+1} )\}
% \end{aligned}
$}
\leftline{
$17.
\{T,\beta\}\
\text{OrderBy}
\begin{aligned}
    \{T_{1} | (\forall \alpha \in T_1,\ \xi_{\alpha} (T_1)=\xi_{\alpha} (T)) 
\wedge(\forall \alpha \in T,\ \xi_{\alpha} (T)=\xi_{\alpha} (T_1))
 \wedge(\forall \alpha_i \in \sigma_{T_1.{\overline{\beta}}}(T_1),\ \alpha_i > \alpha_{i+1} )\}
\end{aligned}
$}
% $$
% \{T,\beta\}\
% ORDER\ BY\ ASC
% \begin{aligned}
%     \{T_{1} | (\forall \alpha \in T_1,\ \xi_{\alpha} (T_1)=\xi_{\alpha} (T)) 
% \wedge(\forall \alpha \in T,\ \xi_{\alpha} (T)=\xi_{\alpha} (T_1))
%  \wedge(\forall \alpha_i \in \sigma_{T_1.{\overline{\beta}}}(T_1),\ \alpha_i < \alpha_{i+1} )\}
% \end{aligned}
% $$
\leftline {\textbf{Logical operation}\\}
\leftline{
$18.
\{\Theta \}
\text{EXISTS}
\begin{aligned}
    \{\Theta_1 | \Theta_1=(\Theta = TRUE)\}
\end{aligned}
\ 19.
\{\Theta_{1}, \Theta_{2}\}
\text{AND}
\begin{aligned}
    \{\Theta |  \Theta=\Theta_{1} \wedge \Theta_{2} \}
\end{aligned}
\ 20.
\{\Theta_{1}, \Theta_{2}\}
\text{OR}
\begin{aligned}
    \{\Theta |  \Theta=\Theta_{1} \vee \Theta_{2} \}
\end{aligned}\ 21.
\{\Theta_{1}\}
\text{NOT}
\begin{aligned}
    \{\Theta |  \Theta = \neg \Theta_{1}\}
\end{aligned}
$}
% \leftline{19.  AND:  $\Theta_1$\ and\ $\Theta_2$ \\ }
% $$\frac{
% \{\Theta_{1}, \Theta_{2}\}
% }{
% \begin{aligned}
%     \{\Theta |  \Theta=\Theta_{1} \wedge \Theta_{2} \}
% \end{aligned}
% }$$
\leftline{
$22.
\{\Theta\}\
\text{IS\ (NOT)\ NULL}
\begin{aligned}
    \{\Theta_1 |  \Theta_1 = (\Theta\ =/\ne\ NULL)\}
\end{aligned}
\ \ \ \ \ \ 23.
\{T,\beta,v_1,v_2\}\
    \text{BETWEEN}
\begin{aligned}
    \{\Theta |  \Theta=(v \in \pi_{\beta}(T), \}
(v \ge v_1) \wedge (v \le v_2))\}
\end{aligned}
$}
% \leftline{21. NOT:  not $\Theta$ \\ }
% $$\frac{
% \{\Theta_{1}\}
% }{
% \begin{aligned}
%     \{\Theta |  \Theta = \neg \Theta_{1}\}
% \end{aligned}
% }$$
% \leftline{23. $\Theta$ IS NOT NULL:  $\Theta$ is not null \\ }
% $$\frac{
% \{\Theta\}\
% }{
% \begin{aligned}
%     \{\Theta_1 |  \Theta_1 = (\Theta\ \ne\ NULL)\}
% \end{aligned}
% }$$
\leftline {\textbf{Join operation}\\}
% $$
% \{T_{1}, T_{2}\}
% NATURAL\ JOIN \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
% \{T_{1}, T_{2}\}
% LEFT\ JOIN \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
% \{T_{1}, T_{2}\}
% RIGHT\ JOIN \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  
% \{T_{1}, T_{2}\}
% FULL\ JOIN 
% $$
% $$
% \begin{aligned}
%     \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta}) 
%     \wedge(\beta \in T_2.\overline{\beta})) \ \ \ \ \ \ \ \ \ 
%     \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee((\beta \in T_1.\overline{\beta}) 
%     \ \ \ \ \ \ \ \ \ \ 
%     \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_2.\overline{\beta})\vee((\beta \in T_1.\overline{\beta})
%     \ \ \ \ \ \ \ \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee(
%     \beta \in T_2.\overline{\beta}))
%  \wedge\\ 
%  \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),
%  \ \ \ \ \ \ \ \ \ \ \wedge(\beta \in T_2.\overline{\beta})))\wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),
%  \ \ \ \ \ \ \ \ \ \ \wedge(\beta \in T_2.\overline{\beta})))
%  \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),
%  \ \ \ \ \ \ \ \ (\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\\
% \xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1)) 
% \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),
% \ \ \ \ \ \ \ \ \ \ \ \xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1)) 
% \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),
% \ \ \ \ \ \ \ \ \ \ \ \ \xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1)) 
% \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\ \ \ \ \ \ \ \ \xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))
% \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),
% \\
% \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
% \ \ \ \ \ \ \ \ \ \ \ \
% \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
% \ \ \ \ \ \ \ \ \ \ \ \ \ 
% \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
% \ \ \ \ \ \ \ \ \ \ 
% \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
% \end{aligned}
% $$
% $$
% \{T,\Theta\}
% ON
% \begin{aligned}
%     \{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1) 
%  \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)
%  \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}
% \end{aligned}
% $$
\leftline{
$24.
\{T_{1}, T_{2}\}
\text{NaturalJoin}
\begin{aligned}
    \{T &| (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta}))
 \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1)) \\
&\wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
$}
\leftline{
$25.
\{T_{1}, T_{2}\}
\text{LeftJoin}
\begin{aligned}
    \{T& | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee((\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta})))
 \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))\\ 
&\wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
$}
\leftline{
$26.
\{T_{1}, T_{2}\}
\text{RightJoin}
\begin{aligned}
    \{T &| (\forall \beta \in T.\overline{\beta},(\beta \in T_2.\overline{\beta})\vee((\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta})))
 \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))\\ 
&\wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
$}
\leftline{
$27.
\{T_{1}, T_{2}\}
\text{FullJoin}
\begin{aligned}
    \{T &| (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee(\beta \in T_2.\overline{\beta}))
 \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))\\
&\wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
$}
\leftline{
$28.
\{T,\Theta\}
\text{ON}
\begin{aligned}
    \{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1) 
 \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)
 \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}
\end{aligned}
$}
\leftline {\textbf{Function operation}\\}
\leftline{29.
$
\{str\}
\text{RTRIM}
\begin{aligned}
    \{str1 | (str1=str[0,|str1|]) 
 \wedge(\forall i \in (|str1|,|str|),str[i]=space) \}
\end{aligned}
$}
\leftline{30.
$
\{str\}
\text{LTRIM}
\begin{aligned}
    \{str1 | (str1=str[|str|-|str1|,|str|])
 \wedge(\forall i \in (0,|str|-|str1|),str[i]=space) \}
\end{aligned}
$}
\leftline{
$31.
\{str,length,str1\}
\text{RPAD}
\begin{aligned}
    \{str2 | (|str2|=length)
\wedge(str2[0,|str|]=str)
 \wedge
 (\forall i \in (|str|,|str2|,
str2[i]=str1[(i-|str|)\%(str1)]) \}
\end{aligned}
$}
\leftline{
$32.
\{str,length,str1\}
\text{LPAD}
\begin{aligned}
    \{&str2 | (|str2|=length) 
 \wedge(str2[|str2|-|str|,|str2|]\\
 &=str) 
\wedge(\forall i \in (0,|str2|-|str|,
str2[i]=str1[i\%|str1|]) \}
\end{aligned}
$}
\leftline{
$33.
\{str,length\}
\text{LEFT}
\begin{aligned}
    \{str1 | str1=str[0,length]\}
\end{aligned}
\ \ \ \ \ \ \ 34.
\{str,length\}
\text{RIGHT}
\begin{aligned}
    \{str1 | str1=str[|str|-length,|str|] \}
\end{aligned}
$}
\leftline{
$35.
\{str1,str2\}
\text{INSTR}
\begin{aligned}
    \{n | str2=str1[n,n+|str2|]
 \wedge(\forall i \in (0,n-1),str1[i,i+|str2|]\ne str2\}
\end{aligned}
$}
% \leftline{locate/position($str1,str2,start$) \\}
\leftline{
$36.
\{str1,str2,start\}
\text{LOCATE/POSITION}
\begin{aligned}
    \{n | str1=str2[n,n+|str1|]
\wedge(\forall i \in (start,n),str2[i,i+|str1|]\ne str1\}
\end{aligned}
$}
% \leftline{substr/substring/mid($str,start,length$) \\ }
\leftline{
$37.
\{str,start,length\}
\text{SUBSTR\ SUBSTRING\ MID}
\begin{aligned}
    \{str1 | str1=str[start,start+length]\}
\wedge(\forall i \in (start,n),str2[i,i+|str1|]\ne str1\}
\end{aligned}
$}
% \leftline{substring_index($str,char,index$) \\ }
\leftline{
$38.
\{str,char,index\}
\text{SUBSTRING\_INDEX}
\begin{aligned}
    \{str1 | str1=str[0,|str1|]
 \wedge(str[|str1|]=index
\wedge(\xi_{char}(str)=index-1\}
\end{aligned}
$}
\leftline{
$39.
\{str\}
\text{REVERSE}
\begin{aligned}
    \{str1 | (|str1|=|str|)
 \wedge(\forall i \in (0,|str|),str[i]=str1[|str1|-i])\}
\end{aligned}
$}
\leftline{
$40.
\{str,start,length,str1\}
\text{INSERT}
\begin{aligned}
    \{&str2 | (str2[0,start]=str[0,start]) 
\wedge
(str2[start+|str1|,
|str2|]
=str[start+length,|str2|])\\
&\wedge(str2[,start,start+
|str1|]=str1
\wedge(|str2|-len(str1=|str|-length)\}
\end{aligned}
$}
\leftline{
$41.
\{str,\overline{str}\}
\text{FIND\_IN\_SET/FIELD}
\begin{aligned}
    \{n | (\overline{str}[n]=str) 
\wedge(\forall i \in (0,n),\overline{str} \ne str)\}
\end{aligned}
$}
\leftline{42.
$
\{index,\overline{str}\}
\text{ELT}
\begin{aligned}
    \{str | (\overline{str}[index]=str)
\wedge(\forall i \in (0,index),\overline{str}[i]\ne str)\}
\end{aligned}
\ \ 43.
\{n\}
\text{SPACE}
\begin{aligned}
    \{str | (|str|=n)\wedge(\forall i \in (0,|str|),str[i]=space)\}
\end{aligned}
$}
\leftline{
$44.
\{str,n\}
\text{REPEAT}
\begin{aligned}
    \{str1 | (|str1|=n*|str|) 
\wedge(\forall i \in (0,|str1|),str1[i]=str[i\%|str|])\}
\end{aligned}
$}
\leftline{
$45.
\{str\}
\text{UPPER(UCASE)/LOWER(LCASE)}
\begin{aligned}
    \{str | (|str|=|str1|)
 \wedge(\forall i \in (0,|str|),str1[i]=ascii(str[i]-/+32))\}
\end{aligned}
$}
\leftline{
$46.
\{char\}
\text{ASCII}
\begin{aligned}
   \{n | n=char+0\} 
\end{aligned}
\ \ \ 47. 
\{n\}
\text{CHAR}
\begin{aligned}
    \{char | char=ascii(n)\}
\end{aligned}
$}
\leftline{
$48. 
\{\Theta,\Theta_{1},\Theta_{2}\}
\text{CASE/IF}
\begin{aligned}
    \{\Theta_{3} | ((\Theta_{3}=\Theta_{1})\wedge(\Theta=TRUE))\vee
((\Theta_{3}=\Theta_{2})\wedge(\Theta=FALSE))\}
\end{aligned}
$}
% $$
% \{\Theta,\Theta_{1},\Theta_{2}\}
% CASE/IF
% \begin{aligned}
%     \{\Theta_{3} | \Theta_{3}=\Theta_{1}, \Theta=TRUE;
% \Theta_{3}=\Theta_{2}, \Theta=FALSE\}
% \end{aligned}
% $$
\leftline{
$49.
\{\Theta_{1},\Theta_{2}\}
\text{NULLIF}
\begin{aligned}
    \{\Theta_{3} | ((\Theta_{3}=NULL)\wedge(\Theta_{1}=\Theta_{2}))\vee 
((\Theta_{3}=\Theta_{1})\wedge(\Theta_{1}\ne \Theta_{2})) \}
\end{aligned}
$}
\leftline{
$50.
\{\overline{str}\}
\text{COALESCE}
\begin{aligned}
    \{n | (\overline{str}[n]=NULL) 
\wedge(\forall i \in (0,n),\overline{str}\ne NULL)\}
\end{aligned}
$}
\leftline {\textbf{Compound semantics}\\}
\leftline{1. SELECT $T.\overline{\beta}$ FROM T\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 2. SELECT $T.\overline{\beta}$ FROM T WHERE $\Theta$ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 3. $T_1,T_2$ Collection Operation $T$\\ }
$\frac{\left\{T\right\}\ \text{FROM}\ \left\{T\right\},\ \left\{T\right\}\ \text{SELECT}\ \overline{\beta}\  \left\{T_{s}\right\}}{\left\{T\right\}\ \text{FROM;\ SELECT}\ \overline{\beta}   \left\{T_{s}\right\}}\ \ \ \ 
    \frac{\left\{T\right\}\ \text{FROM}\ \left\{T\right\},\ \left\{T\right\}\ \text{WHERE}\ \Theta\  \left\{T_w\right\},\left\{T_w\right\}\ \text{SELECT}\ \overline{\beta}\   \left\{T_{sw}\right\}}{\left\{T\right\}\ \text{FROM;\ WHERE}\ \Theta;\ \text{SELECT}\ \overline{\beta}\    \left\{T_{sw}\right\}}\ \ \ \ \{T_1,T_2\}\ \text{Collection\ Operation}\ \{T\}$
~\\
\leftline{4. SELECT $\beta_1$, Aggregation Operation ($T.\beta_2$) FROM T GROUP BY $\beta_1$ HAVING $\Theta$ \\ }
$\frac{\left\{T\right\}\ \text{FROM}\ \left\{T_1\right\},\ \left\{T_1\right\}\ \text{GroupBy}\ \left\{T_2\right\},\ \left\{T_2,\beta_2\right\}\ \text{Agg}\ \left\{x_{agg}\right\},\left\{T_2,\beta_1,\beta_2,x_{agg}\right\}\ \text{SELECT}\ \left\{T_3\right\},\ \left\{T_3,\Theta\right\}\ \text{HAVING}\ \left\{T_4\right\}\ }{\left\{T,\beta_2\right\}\ \text{FROM;\ GroupBy;\ Agg}     \left\{x_{agg}\right\}\left\{T_2,\beta_1,\beta_2,x_{agg}\right\}\ \text{SELECT;\ HAVING;}\     \left\{T_4\right\}}$
% \\ \hspace*{\fill} \\
% $\frac{\left\{T_2,\beta_1\right\}\ ORDER\ BY \left\{T_3\right\} }{\left\{T_2,\beta_1\right\}\ ORDER\ BY;\     \left\{T_3\right\}}$
\\ \hspace*{\fill} \\
\leftline{5. SELECT $T.\beta_1$ FROM T ORDER BY $\beta_1$ ASC/DESC\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 6. SELECT $T\-1.\overline{\beta}$ FROM $T\_1$ Join Operation $T\_2$ \\ } 
$\frac{\left\{T\right\}\ \text{FROM}\ \left\{T_1\right\},\ \left\{T_1,\beta_1\right\}\ \text{SELECT}\ \left\{T_2\right\},\left\{T_2,\beta_1\right\}\ \text{OrderBy} \left\{T_3\right\} \ }{\left\{T,\beta_1\right\}\ \text{FROM;\ SELECT;\ OrderBy;}\left\{T\right\} }$\ \ \ \ \ \ \
$\frac{\left\{T_1,T_2\right\}\ \text{JOIN\ Operation}\ \left\{T\right\},\left\{T\right\}\ \text{FROM}\ \left\{T\right\},\ \left\{T\right\}\ \text{SELECT}\ \overline{\beta}\  \left\{T_{s}\right\}}{\left\{T\right\}\ \text{JOIN\ Operation;\ FROM;\ SELECT}\ \overline{\beta}   \left\{T_{s}\right\}}$
\end{framed}
\caption{Semantic rules for SQL}
\label{fig:semantic1}
}\end{figure*}

==> introduction-old.tex <==
\section{Introduction}
% Database management systems (DBMS), e.g., Oracle\cite{b6}, Access\cite{b14}, MySQL\cite{b1} and PostgreSQL\cite{b15}, offer centralized management and control of databases to ensure their security and integrity and play a vital role in various systems.  
% Representative examples of DBMS include Oracle\cite{b6}, Access\cite{b14}, MySQL\cite{b1} and PostgreSQL\cite{b15}, among others. 
% These modern DBMSs employ different database models to track entities, attributes, and relationships. Among the widely adopted DBMSs for personal computers, mainframes, and servers, relational DBMSs take the lead. In relational databases, data is organized in tables, facilitating efficient storage and retrieval. 

% The practical applications of DBMS span a wide range, with over 4.0 billion users employing embedded DBMSs, and Relational Database Management Systems (RDBMS) being extensively used in numerous websites. 
%Consequently, due to their pervasive adoption, DBMSs have become attractive targets for security attacks. 
%For instance, in 2008, MySQL v5.1 has been found to contain a critical bug where the failure of the partition function may lead to crashes or even data loss \ls{provide reference}. 

%Given their significance, quality assurance is of paramount importance for relational databases, and testing emerges as a crucial quality assurance technique that garners substantial attention. 
%
%Currently, numerous testing techniques are available for ensuring the quality of relational databases. Initially, testing efforts primarily concentrated on detecting crashes in database management systems (DBMS). To accomplish this, random query generators like SQLsmith\cite{b1}\ls{The reference is wrong.} were widely employed to thoroughly test DBMSs. These tools are highly effective in identifying queries that can cause DBMS processes to crash, such as those leading to buffer overflow. 
% Furthermore, fuzzers like AFL\cite{b2} can also be utilized for DBMS testing. These endeavors have proven successful in detecting DBMS crash issues.
% However, our specific focus lies in addressing logical bugs within DBMS. These bugs pertain to errors that result in queries producing incorrect results. Unlike crashes, these errors do not cause the DBMS to malfunction or terminate abruptly, making them considerably more challenging to detect. For a given query, the DBMS may erroneously omit a record from the result set, retrieve a record that should not be included, or calculate an incorrect result for a specific function or operator. Such errors are arduous for users to detect and can easily go unnoticed, particularly given the large scale of many databases.

% \noindent\textbf{Test Oracle Construction} 
%The detection of logical bugs in relational databases primarily relies on the construction of test oracles. One effective approach for constructing test oracles is through the use of differential testing, which has shown promising results. This method detects errors by comparing the results of the same SQL query executed on different DBMSs. However, due to variations in SQL syntax among different systems, these approaches\cite{b12}\cite{b27} can only detect functions with similar syntax in each system, limiting the scope of detection.

% Another successful testing method is based on the construction of metamorphic relations. Several works closely related to this topic include Pivot Query Synthesis (PQS) \cite{b17}, Non-optimized Reference Engine Construction (Norec) \cite{b18}, and Ternary Logical Partitioning (TLP) \cite{b19}. 
%这种方法通过构造语义相同的等价关系，生成一些格式一定的测试用例，通过等价关系得到等价查询，比较两个语义相同的测试用例的返回结果是否相同来检测问题，都取得了很好的效果。
% These approaches, by constructing equivalence relations with identical semantics, generates test cases with specific formats. They compare the results of test cases with identical semantics to detect issues, and it has proven to be highly effective.

% These approaches employ metamorphic relations to detect logical bugs in DBMSs and have achieved significant results.
% PQS\cite{b17} method selects a row of data, constructs a query statement based on that row, and verifies whether the result set contains the selected row. Norec\cite{b18} compares the return values of query statements with those returned by non-optimized DBMSs, successfully identifying numerous logic errors in multiple systems. TLP\cite{b19} provides an automated testing method called query partitioning, which divides a query SQL statement into multiple statements, ensuring that the result sets of the divided statements should be equal to the original statement. By executing these statements, logic errors can be identified if the result sets differ.
% The Sqlright integrates these three methods, incorporating multiple techniques to verify data correctness, and extends the mutation testing based on the three Oracle methods.

However, existing methods for constructing test oracle in DBMS have some limitations.
% For example, PQS cannot detect duplicate rows in the result set as they are not identifiable in this method. NoREC can only detect optimization issues in expressions after the WHERE keyword. TLP has a broader coverage, including group operations, sorting, and other features besides the WHERE keyword. However, the equivalent queries constructed by TLP are both executed by DBMSs that adopt procedural programming methods, which may miss certain inherent logic errors of DBMS.
% In conclusion, the first issue with detection methods based on constructing metamorphic relations is the limitation in the scope of detection. The proposed mutation relations often can only detect specific formats of statements or partial functionalities in Oracle. Constructing test oracles through differential testing is constrained by the implementation differences among different DBMS systems, limiting the testing to functionalities with consistent syntax across different DBMS.
% To address this problem, we parse the test cases into the form of abstract syntax trees, which avoids the syntax limitations encountered in differential testing. 
% In differential testing, if two DBMS have different syntax for the same keyword, a SQL statement containing this keyword may not be executed on both DBMS simultaneously. 
% However, in our method, the parts with different syntax but the same keyword and semantics can still be parsed into two identical abstract syntax trees, and our oracle computation process relies on traversing the abstract syntax tree to invoke keyword semantics, which can support the computation process of any form of SQL statements, overcoming the limitations in the scope of detection in differential testing. 
% The first issue is that existing approaches cannot avoid the inherent problems of imperative programming since both the original queries and the original queries transformed by the metamorphic relations still require execution by the DBMS.

% \lstset{
%  label={lst:plsql-code-demo},
%  tabsize=2,
%  basicstyle=\tt\scriptsize,
%  columns=fixed,       
%  numbers=left,
%  numbersep=3pt,
%  numberstyle=\tiny\color{darkgray},
%  frame=none,
%  backgroundcolor=\color[RGB]{245,245,245},
%  keywordstyle=\bfseries,
%  commentstyle=\it\color[RGB]{0,96,96},
%  stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},
%  showstringspaces=false,
%  language=SQL,
%  morekeywords={FUNCTION, DECLARE, IF, ELSIF, RETURN, FOR, LOOP, LANGUAGE},
% }
% \begin{figure*}[htbp]
% % \centerline{\includegraphics[width=1.02\textwidth,height=0.52\textwidth]{fig1.png}}
% % \caption{Overview of \tool{}}
% % \label{fig:overview}
% % \end{figure*}
% \begin{figure}[t]
% \centering
% \begin{subfigure}{0.45\textwidth}
% % \centerline{\includegraphics[width=0.50\textwidth,height=0.05\textwidth]{A bug on MySQL 8.0.29.png}}
% % select Greatest(mod('-12',-4), mod(-12,-4)); 
%  % --  expected:0, actual:0 @
% \begin{lstlisting}
% select least(mod('-12',-4),mod(-12,-4)); 
%   --expected: 0 @\color{green}{\CheckmarkBold}@, actual:-0 @\color{red}{\XSolidBrush}@
% \end{lstlisting}
% \caption{A bug on MySQL 8.0.29 }
% \label{lst:sublisting-a}
% \end{subfigure}

% \begin{subfigure}{0.45\textwidth}
% % \centerline{\includegraphics[width=0.50\textwidth,height=0.13\textwidth]{The inconsistency caused by bitwise operators when calculating negative numbers on MySQL 8.0.29.png}}
% %SELECT -5 | -4;
%  %  -- PostgreSQL: -1, MySQL: 18446744073709551615
% \begin{lstlisting}
% SELECT 1 > (-5 | -4); 
% --PostgreSQL: 1 @\color{green}{\CheckmarkBold}@,  MySQL: 0 @\color{red}{\XSolidBrush}@
% \end{lstlisting}

% \begin{lstlisting}
% The SQL standard is missing operators 
% on binary data types (BINARY, VARBINARY, BLOB) 
% that allow users to bitwise manipulate values. 
% These operators (with straightforward semantics) are:
% BITAND, BITOR, BITNOT
% @\color{red}{\textit{--ISO/IEC 9075, chapter Foundation,Language Opportunities}}@
% \end{lstlisting}
% \caption{An inconsistency caused by bitwise operators and the corresponding SQL specification descriptions
% % when calculating negative numbers on MySQL and PostgreSQL
% }
% \label{lst:sublisting-b}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
% % \centerline{\includegraphics[width=0.50\textwidth,height=0.13\textwidth]{The inconsistency caused by bitwise operators when calculating negative numbers on MySQL 8.0.29.png}}
% \begin{lstlisting}
% SELECT 'Hello' || NULL;
% -- SQLite: NULL, PostgreSQL: 'Hello'
% \end{lstlisting}
% \begin{lstlisting}
% <binary concatenation> is an operator, ||, 
% that returns a binary string by 
% joining its binary string operands in the order given
% @\color{red}{\textit{--ISO/IEC 9075, chapter Foundation,Binary strings}}@
% \end{lstlisting}
% \caption{An inconsistency caused by binary concatenation when calculating NULL}
% \label{lst:sublisting-c}
% \end{subfigure}
% \caption{Examples of Bugs and Inconsistencies}
% \label{fig:combined}
% \end{figure}

% \tcl{(This is an example of a bug)}
% To illustrate, we discovered a simple bug in MySQL 8.0.29 shown in Fig.\ref{lst:sublisting-a}, which was not detectable using previous Oracle methods. This bug arises from inconsistent results when combining the Least and mod functions. Specifically, when calculating negative string data types, we expected the result to be 0, but the actual result obtained was -0. This bug pertains to the semantics of specific keyword combinations and does not involve query optimization.

% SELECT -5 & -4; 
%    -- expected: -8, actual: 18446744073709551608
% SELECT -5 | -4;
%    -- expected: -1, actual: 18446744073709551615
% SELECT 5 ^ -4;
%    -- expected: -7, actual: 18446744073709551609
% SELECT ~5;
%    -- expected: -6, actual: 18446744073709551610
% SELECT -3 > (5 ^ -4); -- expected: 1, actual: 0
% It is important to note that this bug detection showcases the effectiveness of our keyword semantics, as it highlights issues related to the function's handling of specific inputs.

% The second issue is that the detection methods based on different testing and metamorphic relation cannot identify cases that do not comply with the SQL Specification. In other words, having the same execution results does not guarantee the absence of bugs, as both implementations might violate the SQL Specification. Therefore, to accurately construct test oracles covering all SQL statements, it is essential to start from the semantics defined in the international standard of the SQL language.
% Besides, when the same SQL statement yields inconsistent results on different DBMS, it does not necessarily indicate a bug in a specific system. 
% %由于SQL Specification对一部分功能的描述不清晰，
% Owing to the ambiguous descriptions of certain functionalities in the SQL Specification, two dbms might have different implementation choices for a certain functionality, which is not necessarily an error.
% %但是这对用户使用数据库系统造成了很大的影响，当我们切换数据库使用这些实现不一致的功能时，会得到一些与预期不符的结果，影响我们的使用。
% However, this poses substantial challenges for users of database systems. When transitioning between databases and leveraging these features with inconsistent implementations, unexpected outcomes may arise, hindering our operational efficiency.
% \begin{figure}[htbp]
% % \centerline{\includegraphics[width=0.50\textwidth,height=0.13\textwidth]{The inconsistency caused by bitwise operators when calculating negative numbers on MySQL 8.0.29.png}}
% \begin{lstlisting}
% SELECT -5 & -4; 
%    -- expected: -8, actual: 18446744073709551608
% SELECT -5 | -4;
%    -- expected: -1, actual: 18446744073709551615
% SELECT 5 ^ -4;
%    -- expected: -7, actual: 18446744073709551609
% SELECT ~5;
%    -- expected: -6, actual: 18446744073709551610
% SELECT -3 > (5 ^ -4); -- expected: 1, actual: 0
% \end{lstlisting}
% \caption{The inconsistency caused by bitwise operators when calculating negative numbers on MySQL 8.0.29}
% \label{fig:my_label}
% \end{figure}

%上面这个例子也是一个我们发现MySQL与SQL Specification不符的现象，该问题与位运算符计算负数时的结果表示有关，我们在测试过程中发现，当操作符为负数时，位运算符的结果出现了不一致现象，经过查阅MySQL的文档，MySQL对位运算符的计算过程是先将操作数转化为无符号64位整数的形式，对该形式的数值进行按位操作，得到最终的结果再将其转化为无符号整数的形式。但是SQL Specification中对位运算符计算规定：如果操作数是有符号整数类型（如整数或小数类型），则按位与的结果也将是有符号整数类型。以-5 & -4为例，我们得到的结果应该是-8这个有符号数。

% \tcl{(This is an example of inconsistency resulting from unclear documentation)}
% Fig.\ref{lst:sublisting-b} illustrates a discrepancy we observed between MySQL and the SQL Specification. This issue is related to the representation of results when performing bitwise operations on negative numbers.During our testing process, we discovered inconsistent behavior in the results of bitwise operators when the operands were negative. Upon consulting MySQL documentation, we found that MySQL performs bitwise operations by first converting the operands to the form of an unsigned 64-bit integer, performing the bitwise operation on the converted values, and then converting the final result back to the form of an unsigned integer. Although the SQL specification lacks a functional description of bit signs, we believe that the signedness of the result (signed or unsigned)should match the signedness of the operands: if the operands are signed integer types (such as integer or decimal types), the result of the bitwise AND operation should also be a signed integer type. 
% %我们在发现这个不一致现象后，在PostgreSQL中进行了测试，我们发现PostgreSQL执行这个查询得到的结果与我们的实现是一致的。
% Upon observing this inconsistency, we conducted tests in PostgreSQL. Our findings indicate that the results from PostgreSQL align with our implementation.
% Taking the example of -5 $|$ -4,
% %MySQL先将-5和-4转化为64位无符号数，也就是补码形式，这两个负数的补码之后一到四位不同，分别是1011和1100，前面的数位均为1，在进行按位或操作时，得到的是一个64位都为1的结果，这是-1的补码形式，但是MySQL却返回了这个结果的无符号整数，即18446744073709551615(2^64-1)。我们期望得到的结果-1是一个有符号解释，因为我们认为结果应该与操作数在有无符号的方面保持一致，而MySQL默认将其解释为无符号整数。但是在PostgreSQL中我们得到了预期的有符号数结果。我们认为SQL Specification中没有对位运算符的语义解释清楚，导致了这种各个数据库实现出现不一致的问题，也影响了我们的使用。
% MySQL initially transforms '-5' and '-4' into 64-bit unsigned integers, essentially representing them in their two's complement form. The bitwise representation of these negative numbers diverges only in their last three to four digits, being '1011' and '1100', respectively, while the preceding digits are all set to 1. Engaging in a bitwise OR operation on them yields a 64-bit binary number that consists entirely of ones. Although this represents the two's complement of '-1', MySQL returns it as the unsigned integer '18446744073709551615'($2^{64}-1$) . The anticipated result of '-1' is derived from a signed interpretation, based on the premise that the outcome should maintain consistency with the signness of the operands. By default, however, MySQL interprets it as an unsigned integer. Conversely, in PostgreSQL, the expected signed result is obtained. It is posited that the SQL Specification does not adequately elucidate the semantics of bitwise operators, leading to this inconsistency across various database implementations and subsequently impinging on user experience.

% %这个问题会引发的后续问题如代码第九行所示，我们将位运算符的结果用到后续的比较逻辑运算中，会得到不符合我们预期的结果
% The issue highlighted in this question, as indicated in line three of the code, may lead to subsequent problems. We are using the results of bitwise operators in subsequent logical comparisons, which can produce unexpected outcomes on MySQL and PostgreSQL.

%图c同样是一个由于SQL Specification叙述不准确导致的SQLite和PostgreSQL的不一致现象，||运算符是字符串连接的操作符，SQL Specification缺少对||运算符处理NULL值的功能描述，而SQLite和PostgreSQL在相关功能的实现上出现了不一致现象。在SQLite中，任何字符串与NULL相连接都会返回NULL，而在PostgreSQL中，||操作符会将NULL视为一个空字符串。
% \tcl{(This is an example of inconsistency resulting from unclear documentation)}
% Fig.\ref{lst:sublisting-c} illustrates an inconsistency between SQLite and PostgreSQL, stemming from ambiguous descriptions within the SQL Specification. The '$||$' operator serves as a string concatenation operator. The SQL Specification lacks a clear definition of how the '$||$' operator should handle NULL values, leading to divergent implementations between SQLite and PostgreSQL. Specifically, in SQLite, concatenating any string with NULL invariably returns NULL, whereas in PostgreSQL, the '$||$' operator treats NULL as an empty string.

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.50\textwidth,height=0.07\textwidth]{The inconsistency observed when performing division operations involving string data types on MySQL 8.0.291.png}}
% % \begin{lstlisting}
% % SELECT 1/32;
% %    -- 0.0313
% % SELECT '1'/32; 
% %    -- 0.03125 
% % \end{lstlisting}

% \caption{The inconsistency observed when performing division operations involving string data types on MySQL 8.0.29}
% \label{fig:The inconsistency observed when performing division operations involving string data types on MySQL 8.0.29}
% \end{figure}

% According to the SQL Specification, when performing numerical operations, the operands are converted into a compatible data type for the calculation. However, we have observed an inconsistency when performing division operations with operands of string data type. The results obtained from the division operation differ in the number of decimal places from the results obtained when using the corresponding computable numeric data type for that string type. We consider this to be an inconsistency.

% To address this issue, our implemented oracle strictly adheres to the semantic descriptions of each keyword in the SQL Specification. Through our testing oracle, we have identified 11 cases of inconsistency between the implementations of DBMS and the SQL Specification.

% \noindent\textbf{Test Case Generation} 
% %Currently, there are two main approaches for generating test cases for DBMS testing, namely, generation-based and mutation-based test case generation methods. Generation-based fuzzy testing methods have achieved good results, with SQLsmith[1] being a generation-based DBMS fuzzer that can rapidly generate a large number of semantically correct SQL queries based on predefined AST models. However, it can only generate a limited variety of SQL queries constrained by the generation model's syntax rules (e.g., only SELECT statements). RAGS[3] and Apollo[4] generate test cases based on AST models and SQL syntax. Sqlancer[10] is the most advanced generation-based DBMS fuzzer to date, which formulates grammar rules for different keywords and functionalities to guide test case generation. It has implemented basic functionalities of mainstream DBMS like MySQL and significantly improved functional coverage compared to previous tools.
% % On the other hand, another approach for generating DBMS test cases is the mutation-based method, which has also made progress in system testing[17-24]. Traditional mutation-based fuzzers (e.g., AFL) mutate new test cases through random mutations (e.g., flipping bytes of the original input). They can adapt to testing the functionality of DBMS test libraries like SQLite[11] without the need to construct a generating model in advance. However, mutated test cases often contain numerous semantic errors and cannot trigger the complex behaviors of DBMS. To improve DBMS fuzzing performance, some efforts focus on improving the syntax correctness of mutated SQL queries. Sqirrel[12] proposes to enhance the syntactic correctness of SQL test cases by using AFL-based language validity. It designs an intermediate representation (IR) based on type-based mutations to preserve syntax correctness. Ratel[13] enhances SQL generation robustness by combining SQL dictionaries and grammar-based mutations. It also improves feedback accuracy through binary coverage linking and bijective block mapping to enhance DBMS fuzzing performance.
% %当前SQL测试用例生成的方法主要有基于生成和基于突变的方法，SQLsmith, RAGS, Apollo这些基于生成的工具都是基于预定义的AST模型进行测试用例生成，但是这些早期的生成工具由于模型的语法规则限制，只能覆盖一部分的功能。Sqlancer[10]是目前最先进的基于生成的DBMS模糊器，它制定了不同关键字和功能的语法规则，根据这些语法规则指导测试用例的生成。
% %基于突变的方法中，Bati等人[22]较早的提出查询语句结构变异规则，并采用遗传算法，通过查询结果的反馈指导后续变异。Squirrel通过基于AFL的语言有效性来提高SQL测试用例的句法正确性。它根据SQL语法为基于类型的变异设计了一个中间表示（IR），以保持语法正确性。RATEL[25]是针对企业级数据库管理系统设计的模糊测试工具，该方法在提升覆盖度准确度，提升生成测试输入的鲁棒性等方面做出贡献。
% In the current SQL test case generation methods, there are primarily two approaches: generation-based and mutation-based methods. Tools such as SQLsmith, RAGS, and Apollo are generation-based and rely on predefined Abstract Syntax Tree (AST) models for test case generation. However, these early generation tools are limited by the syntax rules of the model, which restrict their coverage to only a portion of the functionality.

% Among generation-based approaches, Sqlancer[10] stands out as the most advanced DBMS fuzzer. It establishes syntax rules for different keywords and functionalities, which are used to guide test case generation.

% On the other hand, mutation-based methods also exist. Bati et al.[22] proposed early query structural mutation rules and used genetic algorithms to guide subsequent mutations based on query result feedback. Squirrel improves the syntactic correctness of SQL test cases through AFL-based language validity. It designs an intermediate representation (IR) based on type-based mutations to maintain syntax correctness. RATEL[25] is a fuzzy testing tool designed for enterprise-level database management systems. This approach contributes to improving coverage accuracy and generating robustness in test inputs.

% Both of these methods suffer from the problem of generating test cases with low coverage of SQL Specification's keywords and functionalities, leading to insufficient testing of DBMS. To address this issue, we propose three coverage criteria based on our implemented semantics, namely, keyword coverage, rule coverage, and branch coverage, and use these criteria to guide test case generation. Our semantics cover all result-determining keywords defined in the SQL Specification, achieving a coverage rate of 84\%. Rule coverage and branch coverage, based on keyword coverage, complement our tests for different inputs of keywords and combinations of keywords.

% % In summary, mutation-based detection methods fail to overcome the limitations of procedural programming. Constructing test oracles through differential testing is constrained by the specific implementations of different DBMS systems. Inconsistencies in the results obtained from executing the same SQL statement in different systems do not necessarily indicate a bug. It could be a result of different implementation choices for a particular feature. Similarly, identical execution results do not guarantee the absence of bugs, as two queries could exhibit the same problem. Additionally, these methods may not detect cases where the results are the same but violate the SQL specification. Therefore, constructing accurate test oracles covering all SQL statements requires starting from the semantics defined by international standards for the SQL language.

% % Our semantics address three key issues. Firstly, when processing an SQL statement, we parse it into an abstract syntax tree (AST), eliminating syntax barriers between different database management systems (DBMSs). For example, if two databases include a keyword with different syntax, our parsing process ensures that the resulting syntax trees are identical based on the respective DBMS grammar rules. Secondly, our semantics comprehensively cover all deterministic keywords specified in the SQL Specification. Additionally, we introduce three coverage metrics: keyword coverage, rule coverage, and branch coverage. These metrics guide the generation of test cases, improving their coverage. Thirdly, we strictly adhere to the requirements of the SQL Specification during the implementation of our semantics. To ensure the correctness of our semantics, we utilize the Prolog language, which follows an imperative programming approach, thereby avoiding the pitfalls associated with procedural programming during SQL execution.

%我们的方法解决了上面两个问题，首先，针对第一个问题，我们使用Prolog语言实现了一种可执行语义，Prolog语言是一种声明式的语言，而SQL语言的编程方式是命令式的，这使得我们的语义在实现中不太可能出现相同的错误。我们将同一个查询在DBMS和可执行语义中分别执行，将得到的结果进行结果比较来检测bug和不一致现象，规避了命令式编程的弊端，可以检测到一些之前oracle无法检测到的问题。
Our approach addresses both of the aforementioned issues. First, to tackle the first problem, we implemented an executable semantics using the Prolog language. Prolog is a declarative language, while SQL is imperative in nature, which makes it less likely for our semantics to encounter the same errors during implementation. We execute the same query in both the DBMS and the executable semantics, compare the results, and use this comparison to detect bugs and inconsistencies. This approach circumvents the drawbacks of imperative programming and can uncover issues that were previously undetectable, even by Oracle.

%针对第二个问题，我们在实现语义的过程中完全根据SQL Specification中对于关键字的定义、功能描述和语法规则来进行实现，没有参考数据库的其他实现文档，保证了我们的可执行语义是严格符合SQL Specification的。
Regarding the second problem, during the implementation of our semantics, we strictly adhered to the definitions, functional descriptions, and syntax rules of keywords as specified in the SQL Specification. We did not reference any other database implementation documents, ensuring that our executable semantics strictly conform to the SQL Specification.

%在可执行语义的基础上，我们提出了三种覆盖度来指导测试用例的生成，分别是关键字覆盖度，语义规则覆盖度，语义分支覆盖度。这三种覆盖度都是根据语义的实现来定义的，在覆盖度的指导下，我们对生成工具进行了改写，从而对SQL Specification中涉及的功能的测试更加全面。
Building upon the executable semantics, we have introduced three coverage criteria to guide the generation of test cases: keyword coverage, semantic rule coverage, and semantic branch coverage. These three coverage criteria are all defined based on the implementation of semantics. With the guidance of these coverage criteria, we have made modifications to our generation tool, thereby enhancing the comprehensiveness of testing for functionalities specified in the SQL Specification.

To sum up, we present the following contributions in this work. 
\begin{itemize}
\item First-time introduction of database testing based on the SQL Specification
\item Introduction of coverage metrics guided by executable semantics to direct test case generation
\item Testing on four real databases resulted in the discovery of 19 bugs and 11 inconsistencies
\end{itemize}

==> preliminary-old.tex <==
\section{PRELIMINARY}
\subsection{Prolog}
Prolog (Programming in logic) is a logical programming language that focuses on deductive reasoning. It is based on the processing of first-order predicate calculus. Prolog stands out for its simplicity in grammar, expressive power, and unique non-procedural language characteristics, making it highly suitable for representing human thinking and reasoning rules.

The grammatical structure of the Prolog language is straightforward yet exhibits a robust descriptive capability. It comprises three fundamental components: facts, rules, and queries. Facts and rules serve to describe the axioms of a given domain, while queries represent propositions to be proven. In the context of data and relationships, facts and rules provide descriptions, with queries serving as data query statements. Similarly, when facts and rules capture laws governing state changes, queries represent the desired target state.

We will introduce how we implement the semantics of SQL using the Prolog programming language.Taking this SQL statement as an example.

{\tt select\ t1.a\ from\ t1\ where\ t1.b\ >\ 5}
% \begin{equation}\label{eq:rule coverage}
% \begin{aligned}
%     select\ t1.a\ from\ t1\ where\ t1.b\ >\ 5 
% \end{aligned}
% \end{equation}
% The operation is divided into two steps. The first step is to filter eligible data to form a new list.

\lstset{
 label={lst:plsql-code-demo},
 tabsize=2,
 basicstyle=\tt\scriptsize,
 columns=fixed,       
 numbers=left,
 numbersep=3pt,
 numberstyle=\tiny\color{darkgray},
 frame=none,
 backgroundcolor=\color[RGB]{245,245,245},
 keywordstyle=\bfseries,
 commentstyle=\it\color[RGB]{0,96,96},
 stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},
 showstringspaces=false,
 language=SQL,
 morekeywords={FUNCTION, DECLARE, IF, ELSIF, RETURN, FOR, LOOP, LANGUAGE},
}
\begin{figure}[htbp]
% \centerline{\includegraphics[width=0.50\textwidth,height=0.12\textwidth]{Prolog demo -- select.png}}
\begin{lstlisting}
from_clause(T,List,Z) :-
    list(T),
    natural_join(T,List,Z).
from_clause(T,List,Join_type,Z) :-
    list(T),
    Join(T,List,Join_type,Z).
from_clause(T,List,Z) :-
    T =\= list(T),
    table_select(T,List,Z).
table_select(T,[[Th|Ts]|Ls],Ts) :-
    T = Th.
table_select(T,[[Th|Ts]|Ls],Z) :-
    T \= Th,
    table_select(T,Ls,Z).

% select_clause(X,[],[]).
select_clause(NULL,List,[]).
select_clause(X,List,Z) :-
    integer(X),
    add_X(X,List,T),
    select_clause(X,T,Z).
select_clause(X,List,Z) :-
    string(X),
    add_X(X,List,T),
    select_clause(X,T,Z).
select_clause(X,List,Z) :-
    number(X), X =\= integer(X),
    add_X(X,List,T),
    column_select(X,T,Z).
select_clause(X,List,Z) :-
    list(X),
    column_select(X,List,Z).
add_X(X,[L|List],[[X|L]|T]) :-
    add_X(X,List,T).
column_select(X,[H|List],[H|Filtered]) :-
    check_condition(X,H),
    column_select(X,List,Filtered).
column_select(X,[H|List],Filtered) :-
    column_select(X,List,Filtered).
check_condition(X,[[L|Ls]|[R|N]]) :-
    X = L,
    R > 5.
check_condition(X,[[L|Ls]|[R|N]]) :-
    X \= L,
    check_condition(X,[Ls|N]).


from_clause([[t1,[a,b],[1,4],[2,5],[3,8],[4,3],[5,6]],
[t2,[c],[1],[2],[3]]],Table).
--Table = [t1,[a,b],[1,4],[2,5],[3,8],[4,3],[5,6]].

select_clause(t1.b,[t1,[a,b],[1,4],[2,5],[3,8],[4,3],
[5,6]],Filtered).
--Filtered = [[2],[3]]
\end{lstlisting}
\captionsetup{justification=centering}
\caption{Prolog demo -- select}
\label{fig:prolog-demo}
\end{figure}

%我们在fig 3中展示了该语句的prolog语义，分为两个步骤，首先是调用from关键字的语义读入数据表的数据，第二步是调用select的语义筛选出符合条件的数据。
In Figure~\ref{fig:prolog-demo}, we present the Prolog semantics of this statement, which is divided into two steps. The first step involves the semantics of the 'from' keyword, which reads data from a data table. The second step involves the semantics of the 'select' keyword, which filters data that meets the specified conditions.

%我们在给出的代码示例中着重展示了from和select的事实和规则，在这些规则中，还涉及了语义对join关键字和对小于符号的处理，因为这一部分并不是关键的语义，所以我们的代码示例仅仅给出了略写。
In the provided code example, we focus on demonstrating the facts and rules for 'from' and 'select'. Within these rules, there are also considerations for the semantics of the 'join' keyword and the handling of the greater-than symbol ('$>$'). However, since this portion is not a key part of the semantics, our code example provides only a brief outline.

%from_clause和select_clause是处理from表达式和select表达式的主函数，他们分别代表了不同这两个关键字面对不同的输入时的处理情况。每个函数都代表一条规则，函数的最后一个参数代表该函数的返回值，前面的参数代表函数的输入。第1-14行代码是from关键字的语义规则，其中第1-3行代表from的参数是使用逗号连接的多个表的情况(from t1,t2)，输入T代表from的参数，List代表涉及的所有表的信息，包含表中所有的属性和数据。第二行首先判断参数T([t1,t2])是否是一个列表，list是prolog的内置函数，如果是包含多个值的列表，我们在第三行调用natural join的语义对表内容进行连接。第4-6行代表from的参数是包含join的子句的情况(from t1 left join t2)，此时传入的参数包含具体的join类型，我们在调用join语义时也会根据具体的类型进行具体的计算。语义的7-9行代表from的参数是一个表(from t1)，在这种情况下，我们调用table_select函数选择表集合中的t1这个表，将它作为from的返回值返回。
The {\tt from_clause} and {\tt select_clause} are the main functions for processing the 'from' and 'select' expressions, respectively. They represent the handling of these two keywords when dealing with different inputs. Each function represents a rule, with the final parameter of the function representing the return value, and the preceding parameters representing the function's inputs. The code lines 1-14 are the semantic rules for the 'from' keyword. Lines 1-3 handle the case when 'from' has multiple tables separated by commas (e.g., {\tt from t1, t2}). The input 'T' represents the 'from' parameters, and 'List' contains information about all the tables, including their attributes and data. Line 2 checks if the parameter 'T([t1, t2])' is a list (Prolog's built-in 'list' predicate), and if it is, line 3 calls the semantics of a natural join to connect the tables. Lines 4-6 handle the case when 'from' includes a clause with a join (e.g., {\tt from t1 left join t2}). In this case, the input parameters include the specific join type, and the join semantics will be computed based on the specific type. Lines 7-9 handle the case when 'from' has only one table (e.g., {\tt from t1}). In this situation, we call the {\tt table_select} function to select the table 't1' from the table collection and return it as the result of 'from'.

%代码中的16-45行代表了select语义对数据进行筛选的过程。select_clause代表select语义处理的参数的不同规则，代码16-32行分别展示了select语义对null，整数，浮点数，字符串，列引用的处理，如果参数是NULL，那么select的返回值应该是一个空列表。而如果返回值是某个常量，我们会在List中所有的数据里加入一列，而这列的属性和值，都是这个常量。33-34行的add_X函数展示了这个处理过程。在根据不同的参数完成初步处理后，我们调用column_select函数进行数据筛选，第35-37行代表语义在处理列表中的H元素，如果H元素符合第40-45行中check_condition函数的条件，就把H元素加入结果列表，并继续调用select_clause函数对下一个元素进行筛选。第38-39行代表H元素不符合条件，那么语义直接跳过这个元素对剩余列表进行遍历。check_condition相当于是where关键字的语义，X代表条件判断涉及的列，我们首先找到这一列，然后对每个数据进行结果判断。在这个例子中，我们判断的是R这一列的数据大于5的情况。值得注意的是，我们在实际运算时会调用小于号的语义进行计算，该语义有针对不同数据类型运算数的处理情况，但在给出的代码示例中为了突出select和from关键字的语义所以并没有展示出来。
Lines 16-45 in the code represent the process of filtering data in the semantics of the 'select' statement. The {\tt select_clause} handles different rules for the parameters of the 'select' semantics. Lines 16-32 show how the 'select' semantics handle null, integers, floating-point numbers, strings, and column references. If the parameter is NULL, the return value of the 'select' should be an empty list. If the return value is a constant, we add a new column to the 'List' with the same attribute name and value for all rows. Lines 33-34 demonstrate this process using the {\tt add_X} function. After the initial processing based on different parameters, we call the {\tt column_select} function to filter data. Lines 35-37 represent the semantics processing the element H in the list. If the H element meets the conditions in the {\tt check_condition} function shown in lines 40-45, it is added to the result list, and the {\tt select_clause} function continues to filter the next element. Lines 38-39 represent the case where the H element does not meet the condition, and the semantics skip this element and continue iterating through the remaining list. The {\tt check_condition} function is equivalent to the semantics of the 'where' keyword. X represents the column involved in the condition evaluation. We first find this column and then evaluate the condition for each data element. In this example, we are checking if the data in column R is greater than 5. It's worth noting that in actual calculations, the semantics of the greater-than symbol ($>$) would be used for this comparison, which would handle different data types accordingly. However, in the provided code example, the focus is on highlighting the semantics of the 'select' and 'from' keywords, so the details of the greater-than symbol semantics are not shown.

%select_clause是函数名，函数的最后一个参数代表函数的输出，前面的参数代表函数的输入。第2-4行代表语义在处理列表中的H元素，如果H元素符合第7-8行中check_condition函数的条件，就把H元素加入结果列表，并继续调用select_clause函数对下一个元素进行筛选。第5-6行代表H元素不符合条件，那么语义直接跳过这个元素对剩余列表进行遍历。第1行是select的语义跳出递归，返回最终结果的语句。当语义输入为空列表时，即数据列表中的每一条数据都已经筛选完毕，函数返回一个空列表。
% The {\tt select\_clause} is the name of a function, where the last parameter represents the output of the function, and the preceding parameters represent the input. Lines 2-4 represent the semantics processing the H element in the list. If the H element satisfies the conditions specified in lines 7-8 within the check\_condition function, the H element is added to the result list, and the select\_clause function is recursively called to filter the next element. Lines 5-6 represent the case where the H element does not satisfy the condition, and the semantics directly skip this element and proceed to iterate over the remaining list. The first line represents the termination of the select semantics, returning the final result. When the input to the semantics is an empty list, it means that every data in the list has been filtered, and the function returns an empty list.
%该语义的思路是排序方法中的最小值排序算法。第2-4行和第5-7行分别是min_in_list函数在处理列表中的H，K元素，分别调用younger_or_equal和bigger函数进行比较，将比较小的元素保留在列表中作为当前最小值继续与剩余列表中的元素进行比较。语义的第一行代表列表中仅剩一个元素，这个元素就是我们得到的列表中的最小值，我们将该元素作为最终结果返回。

% The second step is to traverse the data in the new list to find the minimum value. 

% \lstset{
%  label={lst:plsql-code-demo},
%  tabsize=2,
%  basicstyle=\tt\scriptsize,
%  columns=fixed,       
%  numbers=left,
%  numbersep=3pt,
%  numberstyle=\tiny\color{darkgray},
%  frame=none,
%  backgroundcolor=\color[RGB]{245,245,245},
%  keywordstyle=\bfseries,
%  commentstyle=\it\color[RGB]{0,96,96},
%  stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},
%  showstringspaces=false,
%  language=SQL,
%  morekeywords={FUNCTION, DECLARE, IF, ELSIF, RETURN, FOR, LOOP, LANGUAGE},
% }
% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.50\textwidth,height=0.11\textwidth]{Prolog demo -- min.png}}
% % \begin{lstlisting}
% % min_in_list([Min],Min).
% % min_in_list([H,K|T],M) :-
% %   younger_or_equal(H,K),
% %   min_in_list([H|T],M). 
% % min_in_list([H,K|T],M) :-
% %   older(H,K),
% %   min_in_list([K|T],M).
% % \end{lstlisting}
% \caption{Prolog demo -- min}
% \label{fig:my_label}
% \end{figure}

% The idea behind this semantics is the minimum value sorting algorithm. Lines 2-4 and 5-7 respectively represent the min\_in\_list function comparing the H and K elements in the list, using the younger\_or\_equal and bigger functions for comparison. The smaller element is kept in the list as the current minimum value and is compared with the remaining elements in the list. The first line of the semantics represents the case where only one element remains in the list, which is the minimum value obtained, and this element is returned as the final result.

%我们可以通过询问的方式获取prolog语义的结果。代码第48-54行代表了询问的过程，我们首先给出t1和t2两张表的信息，以及我们要查询的表名，这个表名我们可以通过解析SQL语句的方式得到，第五十行是from语义给出的答复，我们使用这个结果获取select语义的结果，最终成功得到了指定属性大于5的所有数据。
Inquiry-driven retrieval of Prolog semantics results can be accomplished through the process described in lines 48-54 of the code. Initially, we provide information regarding two tables, namely 't1' and 't2,' along with the target table name to be queried. The determination of this specific table name can be achieved through the parsing of SQL statements. Line 50 signifies the response provided by the 'from' semantics, which serves as the foundation for obtaining the results derived from the 'select' semantics. Consequently, we ultimately achieve the successful retrieval of all data records where the specified attribute exceeds a value of 5.
% With this prolog semantics, we can get the result of a query statement by asking. The following list shows an example. When we expect to get the youngest individual whose level is greater than 5 in the List table, we can get it through the following query: As a result, we first need to parse the data in the data table into a list form, and then pass the list as a parameter into the corresponding semantics, and get the result we want.
% \lstset{
%  label={lst:plsql-code-demo},
%  tabsize=2,
%  basicstyle=\tt\scriptsize,
%  columns=fixed,       
%  numbers=left,
%  numbersep=3pt,
%  numberstyle=\tiny\color{darkgray},
%  frame=none,
%  backgroundcolor=\color[RGB]{245,245,245},
%  keywordstyle=\bfseries,
%  commentstyle=\it\color[RGB]{0,96,96},
%  stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},
%  showstringspaces=false,
%  language=SQL,
%  morekeywords={FUNCTION, DECLARE, IF, ELSIF, RETURN, FOR, LOOP, LANGUAGE},
% }
% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.50\textwidth,height=0.12\textwidth]{Prolog demo -- query and answer.png}}
% % \begin{lstlisting}

% % \end{lstlisting}
% \caption{Prolog demo -- query and answer}
% \label{fig:my_label}
% \end{figure}

% The following example demonstrates a simple family relationship knowledge base containing some facts about family member relationships. We can use Prolog to query and reason about these relationships.

% First, we define some facts and rules:
% The following example reflects the executable semantic features of SQL written by prolog, which is an operation to find the youngest individual with a level greater than 5 in the List table, corresponding to the following SQL statement:

% {\tt select min(age) from List where rank $>$ 5}

% The operation is divided into two steps. The first step is to filter eligible data to form a new list.

% %select_clause是函数名，函数的最后一个参数代表函数的输出，前面的参数代表函数的输入。第2-4行代表语义在处理列表中的H元素，如果H元素符合第7-8行中check_condition函数的条件，就把H元素加入结果列表，并继续调用select_clause函数对下一个元素进行筛选。第5-6行代表H元素不符合条件，那么语义直接跳过这个元素对剩余列表进行遍历。第1行是select的语义跳出递归，返回最终结果的语句。当语义输入为空列表时，即数据列表中的每一条数据都已经筛选完毕，函数返回一个空列表。
% The {\tt select\_clause} is the name of a function, where the last parameter represents the output of the function, and the preceding parameters represent the input. Lines 2-4 represent the semantics processing the H element in the list. If the H element satisfies the conditions specified in lines 7-8 within the check\_condition function, the H element is added to the result list, and the select\_clause function is recursively called to filter the next element. Lines 5-6 represent the case where the H element does not satisfy the condition, and the semantics directly skip this element and proceed to iterate over the remaining list. The first line represents the termination of the select semantics, returning the final result. When the input to the semantics is an empty list, it means that every data in the list has been filtered, and the function returns an empty list.
% \lstset{
%  label={lst:plsql-code-demo},
%  tabsize=2,
%  basicstyle=\tt\scriptsize,
%  columns=fixed,       
%  numbers=left,
%  numbersep=3pt,
%  numberstyle=\tiny\color{darkgray},
%  frame=none,
%  backgroundcolor=\color[RGB]{245,245,245},
%  keywordstyle=\bfseries,
%  commentstyle=\it\color[RGB]{0,96,96},
%  stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},
%  showstringspaces=false,
%  language=SQL,
%  morekeywords={FUNCTION,  IF, ELSIF, RETURN, FOR, LOOP, LANGUAGE},
% }
% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.50\textwidth,height=0.15\textwidth]{the fact and the rule in prolog.png}}
% % \begin{lstlisting}
% % % Facts: Declare the family member relationships
% % father(john, jim).
% % father(john, ann).
% % mother(mary, jim).
% % mother(mary, ann).

% % % Rules: Define parent relationship
% % parent(X, Y) :- father(X, Y).
% % parent(X, Y) :- mother(X, Y).
% % \end{lstlisting}
% \captionsetup{justification=centering}
% \caption{The fact and the rule in prolog}
% \label{fig:the fact and the rule in prolog}
% \end{figure}
% % %该语义的思路是排序方法中的最小值排序算法。第2-4行和第5-7行分别是min_in_list函数在处理列表中的H，K元素，分别调用younger_or_equal和bigger函数进行比较，将比较小的元素保留在列表中作为当前最小值继续与剩余列表中的元素进行比较。语义的第一行代表列表中仅剩一个元素，这个元素就是我们得到的列表中的最小值，我们将该元素作为最终结果返回。

% % The second step is to traverse the data in the new list to find the minimum value. 

% % The idea behind this semantics is the minimum value sorting algorithm. Lines 2-4 and 5-7 respectively represent the min\_in\_list function comparing the H and K elements in the list, using the younger\_or\_equal and bigger functions for comparison. The smaller element is kept in the list as the current minimum value and is compared with the remaining elements in the list. The first line of the semantics represents the case where only one element remains in the list, which is the minimum value obtained, and this element is returned as the final result.
% % \lstset{
% %  label={lst:plsql-code-demo},
% %  tabsize=2,
% %  basicstyle=\tt\scriptsize,
% %  columns=fixed,       
% %  numbers=left,
% %  numbersep=3pt,
% %  numberstyle=\tiny\color{darkgray},
% %  frame=none,
% %  backgroundcolor=\color[RGB]{245,245,245},
% %  keywordstyle=\bfseries,
% %  commentstyle=\it\color[RGB]{0,96,96},
% %  stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},
% %  showstringspaces=false,
% %  language=SQL,
% %  morekeywords={FUNCTION, DECLARE, IF, ELSIF, RETURN, FOR, LOOP, LANGUAGE},
% % }
% % \begin{figure}[htbp]
% % \centering
% % \begin{lstlisting}
% % min_in_list([Min],Min).
% % min_in_list([H,K|T],M) :-
% %   younger_or_equal(H,K),
% %   min_in_list([H|T],M). 
% % min_in_list([H,K|T],M) :-
% %   older(H,K),
% %   min_in_list([K|T],M).
% % \end{lstlisting}
% % \caption{prolog demo -- min}
% % \label{fig:my_label}
% % \end{figure}

% % With this prolog semantics, we can get the result of a query statement by asking. The following list shows an example. When we expect to get the youngest individual whose level is greater than 5 in the List table, we can get it through the following query: As a result, we first need to parse the data in the data table into a list form, and then pass the list as a parameter into the corresponding semantics, and get the result we want.
% % \lstset{
% %  label={lst:plsql-code-demo},
% %  tabsize=2,
% %  basicstyle=\tt\scriptsize,
% %  columns=fixed,       
% %  numbers=left,
% %  numbersep=3pt,
% %  numberstyle=\tiny\color{darkgray},
% %  frame=none,
% %  backgroundcolor=\color[RGB]{245,245,245},
% %  keywordstyle=\bfseries,
% %  commentstyle=\it\color[RGB]{0,96,96},
% %  stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},
% %  showstringspaces=false,
% %  language=SQL,
% %  morekeywords={FUNCTION, DECLARE, IF, ELSIF, RETURN, FOR, LOOP, LANGUAGE},
% % }
% % \begin{figure}[htbp]
% % \centering
% % \begin{lstlisting}
% % select_clause([[1001,4,28],[1002,5,35],[1003,8,26],
% % [1004,3,35],[1005,6,48],[1007,4,19],[1008,6,27],
% % [1009,7,38]],Filtered).
% % --Filtered = [[1003, 8, 26],[1005, 6, 48],
% % [1008, 6, 27],[1009, 7, 38]].
% % min_in_list([[1003, 8, 26],[1005, 6, 48],
% % [1008, 6, 27],[1009, 7, 38]],Min).
% % --Min = [1003, 8, 26]
% % \end{lstlisting}
% % \caption{prolog demo -- query and answer}
% % \label{fig:my_label}
% % \end{figure}

% % \begin{figure}[htbp]
% % \centering
% % \begin{lstlisting}

% % SELECT + 列引用 + FROM + 表引用
% % SELECT + 列引用 + FROM + 表连接
% % SELECT + 列引用 + FROM + 子查询
% % SELECT + 子查询 + FROM + 表引用
% % SELECT + 子查询 + FROM + 表连接
% % SELECT + 子查询 + FROM + 子查询
% % \end{lstlisting}
% % \caption{prolog demo -- query and answer}
% % \label{fig:my_label}
% % \end{figure}

% In the provided code, we define some facts about family member relationships. For example, "john" is the father of "jim" and "ann."Next, we define a rule. parent(X, Y) represents "X is the parent of Y," and it uses father(X, Y) and mother(X, Y) as conditions. This way, Prolog performs logical reasoning based on these facts and rules.

% We can perform some queries and reasoning. For example, we can ask, "Who are the parents of 'jim'?"

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.50\textwidth,height=0.03\textwidth]{the query in prolog.png}}
% % \begin{lstlisting}
% % ?- parent(X, jim).
% % - X = john.
% % \end{lstlisting}
% \captionsetup{justification=centering}
% \caption{The query in prolog}
% \label{fig:the query in prolog}
% \end{figure}

% Prolog will search the facts and rules, finding results that match the query. In this case, Prolog will answer X = john, meaning "john is the father of jim."

Prolog is a great specification language for our use for a number of reasons:
\begin{itemize}
\item It is largely intuitive and convenient (i.e. by specifying rules and facts).
\item It supports various list operations and mathematical expressions, which help to capture semantics involving database operations.
\item It supports automatic reasoning, which is crucial for our purposes.
\item It is a well-studied declarative programming language that is fundamentally different from imperative programming used to control databases. This makes our semantics less likely to have the same errors in implementation.
\end{itemize}



==> references.tex <==
% \begin{thebibliography}{00}

% \bibitem{b2}SQLite. https://www.sqlite.org/index.html. Accessed Nov 2023.
% \bibitem{b3}DuckDB. https://duckdb.org. Accessed Nov 2023.
% \bibitem{b4}McMinn, P., Wright, C. J., McCurdy, C. J.,  Kapfhammer, G. M. (2017). Automatic detection and removal of ineffective mutants for the mutation analysis of relational database schemas. IEEE Transactions on Software Engineering, 45(5), 427-463.
% \bibitem{b5}MariaDB. https://www.mariadb.org. Accessed Nov 2023.
% \bibitem{b6}Oracle. https://www.oracle.com. Accessed Nov 2023.
% \bibitem{b7}Shah, S., Sudarshan, S., Kajbaje, S., Patidar, S., Gupta, B. P.,  Vira, D. (2011, April). Generating test data for killing SQL mutants: A constraint-based approach. In 2011 IEEE 27th International Conference on Data Engineering (pp. 1175-1186). IEEE.
% \bibitem{b8} Liang, Y., Liu, S.,  Hu, H. (2022). Detecting Logical Bugs of {DBMS} with Coverage-based Guidance. In 31st USENIX Security Symposium (USENIX Security 22) (pp. 4309-4326).
% \bibitem{b9} Fu, J., Liang, J., Wu, Z., Wang, M., Jiang, Y. (2022, October). Griffin: Grammar-free DBMS fuzzing. In Proceedings of the 37th IEEE/ACM International Conference on Automated Software Engineering (pp. 1-12).
% \bibitem{b10}Hoare, T. (2003). The verifying compiler: A grand challenge for computing research. Journal of the ACM (JACM), 50(1), 63-69.
% \bibitem{b11}SQLancer. https://github.com/sqlancer/sqlancer. Accessed Feb 2022.
% \bibitem{b12}Slutz, D. R. (1998, August). Massive stochastic testing of SQL. In VLDB (Vol. 98, pp. 618-622).
% \bibitem{b13}Zhu, X., Wen, S., Camtepe, S.,  Xiang, Y. (2022). Fuzzing: a survey for roadmap. ACM Computing Surveys (CSUR), 54(11s), 1-36.
% \bibitem{b14}Access. https://www.microsoft.com/en-us/microsoft-365/access
% \bibitem{b15}PostgreSQL. https://www.postgresql.org. Accessed Nov 2023.
% \bibitem{b16}TiDB. https://www.pingcap.com/tidb/. Accessed Nov 2023.
% \bibitem{b17}Rigger, M.,  Su, Z. (2020). Testing database engines via pivoted query synthesis. In 14th USENIX Symposium on Operating Systems Design and Implementation (OSDI 20) (pp. 667-682).
% \bibitem{b18}Rigger, \vspace{0mm} M. and Su, Z., 2020, November. Detecting optimization bugs in database engines via non-optimizing reference engine construction. In Proceedings of the 28th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering (pp. 1140-1152).
% \bibitem{b19}Rigger, \vspace{0mm}M., Su, Z. (2020). Finding bugs in database systems via query partitioning. Proceedings of the ACM on Programming Languages, 4(OOPSLA), 1-30.
% ghit2020sparkfuzz
% \bibitem{b20}Ghit, B., Poggi, N., Rosen, J., Xin, R., Boncz, P. (2020, June). SparkFuzz: Searching correctness regressions in modern query engines. In Proceedings of the workshop on Testing Database Systems (pp. 1-6).
% chen2020testing
% \bibitem{b21}Chen, X., Wang, C., Cheung, A. (2020, June). Testing query execution engines with mutations. In Proceedings of the workshop on Testing Database Systems (pp. 1-5).
% \bibitem{b22}Bati, H., Giakoumakis, L., Herbert, S., Surna, A. (2007, September). A genetic approach for random testing of database systems. In Proceedings of the 33rd international conference on Very large data bases (pp. 1243-1251).
% \bibitem{b23}Zhong, R., Chen, Y., Hu, H., Zhang, H., Lee, W., Wu, D. (2020, October). Squirrel: Testing database management systems with language validity and coverage feedback. In Proceedings of the 2020 ACM SIGSAC Conference on Computer and Communications Security (pp. 955-970).
% \bibitem{b24}Song, M. (2021, September). Optimization Research on Initial Seeds of the Database Management Systems Fuzzing Framework Squirrel. In Journal of Physics: Conference Series (Vol. 2010, No. 1, p. 012069). IOP Publishing.
% \bibitem{b25}Wang, M., Wu, Z., Xu, X., Liang, J., Zhou, C., Zhang, H., Jiang, Y. (2021, May). Industry practice of coverage-guided enterprise-level DBMS fuzzing. In 2021 IEEE/ACM 43rd International Conference on Software Engineering: Software Engineering in Practice (ICSE-SEIP) (pp. 328-337). IEEE. 
% castelein2018search
% \bibitem{b26}Castelein, J., Aniche, M., Soltani, M., Panichella, A., van Deursen, A. (2018, May). Search-based test data generation for SQL queries. In Proceedings of the 40th international conference on software engineering (pp. 1220-1230).
% ceri1985translating
% \bibitem{b27}Ceri, S., Gottlob, G. (1985). Translating SQL into relational algebra: Optimization, semantics, and equivalence of SQL queries. IEEE Transactions on software engineering, (4), 324-345.
% van2009translating
% \bibitem{b28}Van den Bussche, J., Vansummeren, S. (2009). Translating SQL into the relational algebra. Course notes, Hasselt University and Université Libre de Bruxelles.
% negri1991formal
% \bibitem{b29}Negri, M., Pelagatti, G., Sbattella, L. (1991). Formal semantics of SQL queries. ACM Transactions on Database Systems (TODS), 16(3), 513-534.
% chu2017cosette
% \bibitem{b30}Chu, S., Wang, C., Weitz, K., Cheung, A. (2017, January). Cosette: An Automated Prover for SQL. In CIDR.
% chu2017hottsql
% \bibitem{b31} Chu, S., Weitz, K., Cheung, A., Suciu, D. (2017). HoTTSQL: Proving query rewrites with univalent SQL semantics. ACM SIGPLAN Notices, 52(6), 510-524.
% malecha2010toward
% \bibitem{b32}Malecha, G., Morrisett, G., Shinnar, A., Wisnesky, R. (2010, January). Toward a verified relational database management system. In Proceedings of the 37th annual ACM SIGPLAN-SIGACT symposium on Principles of programming languages (pp. 237-248). 
% veanes2010qex
% \bibitem{b33}Veanes, M., Tillmann, N., De Halleux, J. (2010). Qex: Symbolic SQL query explorer. In Logic for Programming, Artificial Intelligence, and Reasoning: 16th International Conference, LPAR-16, Dakar, Senegal, April 25–May 1, 2010, Revised Selected Papers 16 (pp. 425-446). Springer Berlin Heidelberg. 
% chinaei2007ordered
% \bibitem{b34}Chinaei, H. R. (2007). An Ordered Bag Semantics for SQL (Master's thesis, University of Waterloo).
% ricciotti2022formalization
% \bibitem{b35}Ricciotti, W., Cheney, J. (2022). A Formalization of SQL with Nulls. Journal of Automated Reasoning, 66(4), 989-1030.
% guagliardo2017formal
% \bibitem{b36}Guagliardo, P., Libkin, L. (2017). A formal semantics of SQL queries, its validation, and applications. Proceedings of the VLDB Endowment, 11(1), 27-39. 
% benzaken2019coq
% \bibitem{b37}Benzaken, V., Contejean, E. (2019, January). A Coq mechanised formal semantics for realistic SQL queries: formally reconciling SQL and bag relational algebra. In Proceedings of the 8th ACM SIGPLAN International Conference on Certified Programs and Proofs (pp. 249-261).
% zhou2020symbolic
% \bibitem{b38}Zhou, Q., Arulraj, J., Navathe, S., Harris, W., Wu, J. (2020). A Symbolic Approach to Proving Query Equivalence Under Bag Semantics. arXiv preprint arXiv:2004.00481.
% cheney2021comprehending
% \bibitem{b39}Cheney, J., Ricciotti, W. (2021, August). Comprehending nulls. In The 18th International Symposium on Database Programming Languages (pp. 3-6).
% \bibitem{b40}Zhou, C., Frankl, P. (2012, April). Empirical studies on test effectiveness for database applications. In 2012 IEEE Fifth International Conference on Software Testing, Verification and Validation (pp. 61-70). IEEE.





% \end{thebibliography}

==> semantics.tex <==
\section{Formal Semantics for SQL}

% This work requires the formulation of semantics based on the functional descriptions of keywords in the SQL specification, necessitating the establishment of preconditions and postconditions for various SQL operations.

% In this section, we first presented some fundamental definitions, including symbols for databases, tables, attributes, and data, as well as the definitions of basic operations for retrieval. Building upon these definitions, we then established the formal semantics for keywords.

%在这部分中，我们首先介绍了一些基础定义，包括一些对数据库，表，属性，数据的符号定义和对一些检索时的基本操作的定义。在这些定义的基础上，我们定义了关键字的形式化语义。
\subsection{basic notations}

%在基础定义部分中，我们首先定义了数据库模式，数据库和表的抽象符号，之后我们定义了对表的两项基本操作，取行和取列，我们可以通过这两项操作定位到一个具体的数据。
Table~\ref{table:basic} are the basic notations that are defined in our approach. 
% we initially defined abstract symbols for database schema, database, and tables. Subsequently, we introduced two fundamental operations on tables, namely, retrieving rows and retrieving columns. These operations allow us to locate specific data within a table.
%接下来我们对数据库实例进行了定义，首先定义了数据库，表，表中数据和列属性的实例，之后在取行和取列操作的基础上结合表，属性的实例进行了更具体的定义。
% we proceeded with the definition of database instances. 
% we start by defining instances of databases, tables, data within the tables, and attributes of columns. Building upon the operations of data projection and selection, we further refine the definitions retrieving rows and columns by incorporating concrete instances of tables and attributes. We use $\xi$ express the data or attribute number in the table.
%SQL语句的输入来自表中的数据，但在处理SQL语句的过程中，我们需要处理表达式，我们定义了表达式的种类，首先是数据，我们结合SQL Specification和我们的Prolog语义实现给出了四种数据类型的数据定义，分别是常数(包含整数和浮点数)，布尔类型，字符串类型和字符类型。其次是null的语义，null在SQL中代表未知，是SQL执行过程中需要单独处理的数据类型。第三种就是各种逻辑表达式，我们在下面的的关键字语义中会对各种逻辑运算符进行详细的定义，在基础定义中，我们引入了与，或，非的基本运算。

% % In the process of handling SQL statements, the inputs are derived from the data within the tables. 
% To effectively process SQL statements, we also need to handle expressions. For this purpose, we have defined various types of expressions. First, we have data expressions, which include four data types based on SQL Specification. These data types are constants (including integers and floating-point numbers), booleans, strings, and characters.We use $v$ express the value of the data and use $len()$ express the length of the value. 
% Next, we have defined the semantics for null values. 
% % In SQL, null represents unknown data and requires special handling during the execution process. 
% Lastly, we have addressed various logical expressions. 
% % Detailed definitions for logical operators will be presented in the subsequent section on keyword semantics. 
% % In the foundational definitions, 
% We have introduced basic operations such as $\wedge$, $\vee$, and $\neg$.These three symbols represent set operations of intersection, union, and complement.

% In the context of basic semantics for databases, we initially define the database schema, symbols representing databases, and data tables. On the basis of these three definitions, we also defined constants, lists, sets, and operations for data retrieval such as getting the rows or columns in the data table. The second part in Table I pertains to the definition and manipulation of database instances, which represent the actual data present in the data tables. In this section of the definition, we combine the concrete data instances with the foundational definitions described earlier to facilitate the process of writing the semantics for specific keywords.Lastly, Table II covers the fundamental definition of conditional statements for decision-making processes.In the process of SQL execution, the results obtained are not limited to specific single or multiple data records. They can also include other data types such as boolean data types and NULL values. Additionally, for the convenience of representing semantics, we introduce basic operations for sets, including union, intersection, and complement.
\begin{table}[t]   
\begin{center}   
\caption{Symbol Notations}  
\label{table:basic} 
\begin{tabular}{cccc}   
\hline   \textbf{Symbol} & \textbf{discription} \\     
\hline   D & a database instance  \\
T & a table instance \\
% \multirow{2}*{T} & a table instance \\
% &contains attributes and values T=$(\overline{\beta},\overline{\alpha})$  \\ 
$ \alpha$ & \ls{a data in a data table}  \\ 
$ \overline{\alpha}$ & bags of data  \\
$ \beta$ & attribute  \\
$ \overline{\beta}$ & \ls{bags of attributes}  \\
$ T.\beta_i$ & attribute i in T, i $\in\ Z_{+} $  \\
$ T.\overline{\beta}$ & $T.(\beta_1,...,\beta_k)=(T.\beta_1,...,T.\beta_k)$  \\
% &L(T) & the bag of all attributes of the data table\ T  \\
% &V(T) & the bag of all datas of the data table\ T  \\
$ \pi_{\beta_{i}}(T)$ & the data for attribute i,  i $\in Z_{+}$  \\
$ \sigma_{\Theta}(T)$ & the data that meets the conditions $\Theta$  \\
\multirow{2}*{$ \xi_{\alpha_i}(T)$} & the number of \\
& a data $\alpha_i$ in table T, i $\in Z_{+}$  \\
\multirow{2}*{$ \xi_{\beta_i}(T)$} & the number of \\
& an attribute $\beta_i$ in table T, i $\in Z_{+}$  \\
$v$ & the\ value\ of\ the\ data\\
$len(v)$ & the length of the value \\
$null$ & unknown\ data \\
% $\wedge$ & and \\
% $\vee$ & or \\
% $\neg$ & not \\
$ \Theta $ & v\ $|$\ null\ $|$\ logic\ expression\\
% $c$ & constant,include\ integer\ and\ float \\
% $boolean$   & TRUE\ $|$\ FALSE \\
% $str$ &  String\ type\\
% $char$ &  character\ type\\
\hline   
\end{tabular}   
\end{center}   
\end{table}
% \begin{framed}
% \leftline{$ \Theta(expression): \\ $}
% $$ \left\{
% \begin{aligned}
% &v,&t&he\ value\ of\ the\ data\ \\
% nu&ll,&u&nknown\ data \\
% logic\ ex&pression,&\Theta&\wedge \Theta\ |\ \Theta \vee \Theta\ | \neg \Theta \\
% \end{aligned}
% \right.
% $$
% $$ v=\left\{
% \begin{aligned}
% c,\    & constant,include\ integer\ and\ float \\
% boolean,\   & TRUE\ |\ FALSE \\
% str,\ &  String\ type\\
% char,\ &  character\ type\\
% \end{aligned}
% \right.
% $$
% % \leftline{$ P(predicate): \\ $}
% % $$ P(t_1,...,t_k)=\left\{
% % \begin{aligned}
% % T,\    & (P(t_1,...,t_k))\wedge \\
% %      &  (\forall i \in (1, ...,k),\ t_i != NULL)\\
% % F,\   & (!(P(t_1,...,t_k)))\wedge \\
% %      &  (\forall i \in (1, ...,k),\ t_i != NULL)\\
% % U,\ & \exists i \in (1, ...,k),\ t_i = NULL \\
% % \end{aligned}
% % \right.
% % $$
% % $$ t\ IN\ \overline{t}=\left\{
% % \begin{aligned}
% % T,\    &  \exists i \in (1, ...,k),\ t = t_i \\
% % F,\   &  \forall i \in (1, ...,k),\ t != t_i\\
% % U,\ & (\exists i \in (1, ...,k),\ t_i = NULL)\wedge\\
% % & (\forall i \in (1, ...,k),(t !=t_j) \wedge (t_j!=NULL)) \\
% % \end{aligned}
% % \right.
% % $$
% \end{framed}
\subsection{keyword semantic}
% In the section of keyword semantics, we implemented it based on SQL Specification. 

% Referring to the method proposed by Hoare\cite{b41}, a pair of formulas are placed before and after the corresponding program segment, which are called the precondition and postcondition of the program segment respectively.\\
We adopt the format of Hoare triple~\cite{b41}, shown in Formula~(\ref{eq:hoaretriple}).  
\textit{P} and \textit{Q} are assertions in predicate logic, \textit{P} is the precondition, \textit{Q} is the postcondition and \textit{C} is the command. 
When the evaluation to the precondition \textit{P} is true, executing command \textit{C} establishes the postcondition \textit{Q}. 

\begin{equation}
\label{eq:hoaretriple}
 \{P\} C \{Q\}\\    
\end{equation}

% If the condition pre is established before the execution of program P (the environment at that time meets pre), the condition post must be established in the environment when the execution of program P terminates.

We conducted a statistical analysis of the keywords included in the SQL specification, resulting in a total of 138 keywords. We have implemented the semantics for 116 of these keywords. For the keywords where we were unable to implement the semantics, there are two scenarios. The first scenario is when the keyword's returned results exhibit uncertainty. For instance, functions like "random" and certain time-related functions yield results with a certain level of randomness, while the results of certain window functions are influenced by pagination and result sorting, making deterministic result comparisons infeasible. The second scenario arises when there are differences in the implementation of keywords across different databases. This primarily applies to certain data type conversion functions, as the precision and formatting of data may differ after type conversion, leading us to omit the implementation of such functions.

% We listed the pre conditions and post conditions of the keywords we implemented.The preconditions of the keywords represent the conditions that the input data should satisfy, while the postconditions represent the conditions that the output data should satisfy. We used these conditions to verify the correctness of keyword semantics.
%我们将关键字分为以下类别：查询表达式的基础关键字，集合操作关键字，聚合函数，组操作关键字，条件关键字，表连接关键字，函数关键字

We categorize keywords into the following groups: basic keywords for query expressions, set operation keywords, aggregate functions, grouping operation keywords, conditional keywords, table join keywords, and function keywords.
\begin{spacing}{0.5}
{\scriptsize
\begin{framed}
\leftline {\textbf{Query expression}\\}
~\\
\leftline {1. FROM: from T\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 2. SELECT: select\ $T.\overline{\beta}$\\}
$$\frac{\{T\}}{\{T_1| T_1=T\}}\ \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ \frac{\{T,\overline{\beta}\}}{\{T_1|T_1=\{\pi_{\overline{\beta}}(T)\}\}}$$
% \leftline {2. SELECT: select\ $T.\overline{\beta}$\\}
% $$
% \frac{\{T,\overline{\beta}\}}{\{T_1|T_1=\{\pi_{\overline{\beta}}(T)\}\}}
% $$
\leftline {3. WHERE: where\ $\Theta$\\}
$$\frac{
\begin{aligned}
\{T,\Theta\}
\end{aligned}
}{
\begin{aligned}
\{T_1 | (\forall \alpha \in \sigma_\Theta (T),&\alpha \in T_{1}) 
\wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_{1})\\
&\wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\}
\end{aligned}
}$$
\end{framed}

\begin{framed}
\leftline {\textbf{Collection operation}\\}
~\\
\leftline{4. UNION: T1 union T2 \\ }
$$\frac{
    \left\{T_{1}, T_{2}\right\}
}{
\begin{aligned}
    \{T | (\forall &\alpha_{1} \in T_1,\forall \alpha_{2} \in T_2,  
 \alpha_{1} , \alpha_{2} \in T) \wedge(\forall \alpha_{3} \in T,
\\
(\alpha_{3} \in & T_1)\vee(\alpha_{3} \in T_2))
 \wedge (\forall \alpha_4 \in T,\ \xi_{\alpha_4}(T)=1)\}
\end{aligned}
}$$
\\ \hspace*{\fill} \\
\leftline{5. INTERSECT: T1 intersect T2 \\ }
$$\frac{
    \{T_{1}, T_{2}\}\
}{
\begin{aligned}
    \{T | (\forall \alpha_{1} \in T_1,
 ((\alpha_{1}  \in T_2) \wedge (\alpha_{1}  \in T)) 
 \vee ((\alpha_{1}  \notin  T) \wedge (\alpha_{1}  \notin T_2)))\\
 \wedge(\forall \alpha_{2} \in T,
(\alpha_{2} \in  T_1)\vee(\alpha_{2} \in T_2))
 \wedge (\forall \alpha_3 \in T,\ \xi_{\alpha_3}(T)=1)\}
\end{aligned}
} $$
\\ \hspace*{\fill} \\
\leftline{6. EXCEPT: T1 except T2 \\ }
$$\frac{
    \{T_{1}, T_{2}\}
}{
\begin{aligned}
    \{T | (\forall \alpha_{1}& \in T_1, 
 ((\alpha_{1}  \in T) \wedge (\alpha_{1}  \notin T_2) 
 \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \in T_2)))\\
 &\wedge(\forall \alpha_{2} \in T,(\alpha_{2} \in T_1))
 \wedge (\forall \alpha_3 \in T,\ \xi_{\alpha_3}(T)=1)\}
\end{aligned}
}$$
\\ \hspace*{\fill} \\
\leftline{7. UNION ALL: T1 union all T2 \\ }
$$\frac{
    \{T_{1}, T_{2}\}
}{
\begin{aligned}
    \{T | (\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2,
 \alpha_{1} , \alpha_{2} \in T) 
 \wedge(\forall \alpha_{3} \in T,
(\alpha_{3} \in T_1)
\\
\vee(\alpha_{3} \in T_2))
 \wedge (\forall \alpha_4 \in T,
 \xi_{\alpha_4}(T)=\xi_{\alpha_4}(T_1)+\xi_{\alpha_4}(T_2))\}
\end{aligned}
}$$
\\ \hspace*{\fill} \\
\leftline{8. INTERSECT ALL: T1 intersect all T2 \\ }
$$\frac{
\{T_{1}, T_{2}\}
}{
\begin{aligned}
    \{&T | (\forall \alpha_{1} \in T_1, 
((\alpha_{1}  \in T_2) \wedge (\alpha_{1}  \in T) 
\vee ((\alpha_{1}  \notin T) \\
\wedge (\alpha_{1}  &\notin T_2)))\}
 \wedge (\forall \alpha_2 \in T,\ 
\xi_{\alpha_2}(T)=min(\xi_{\alpha_2}(T_1),\xi_{\alpha_2}(T_2)))\}
\end{aligned}
}$$
\\ \hspace*{\fill} \\
\leftline{9. EXCEPT ALL: T1 except all T2 \\ }
$$\frac{
\{T_{1}, T_{2}\}
}{
\begin{aligned}
    \{T | (\forall \alpha_{1}& \in T_1,
((\alpha_{1}  \in T) \wedge (\alpha_{1}  \notin T_2) 
 \vee ((\alpha_{1}  \notin T) \wedge  (\alpha_{1}  \in T_2)))\}\\
 &\wedge (\forall \alpha_2 \in T,
 \xi_{\alpha_2}(T)=max(\xi_{\alpha_2}(T_1)-\xi_{\alpha_2}(T_2)),0)\}
\end{aligned}
}$$
\end{framed}
\begin{framed}
\leftline {\textbf{Aggregation operation}\\}
~\\
\leftline{10. MIN: min($T.\beta$) \\ }
$$\frac{
\{T,\beta\}
}{
\begin{aligned}
    \{
x_{min} | (x_{min} \in \pi_{\beta}(T),
 \Theta=(v \in \pi_{\beta}(T)\wedge(v < x_{min})),\ \sigma_{\Theta}(T)=\oslash \}
\end{aligned}
}$$

\leftline{11. MAX: max($T.\beta$) \\ }
$$\frac{
\{T,\beta\}
}{
\begin{aligned}
    \{x_{max} | (x_{max} \in  \pi_{\beta}(T), 
\Theta=(v \in \pi_{\beta}(T) \wedge(v > x_{max})),\ \sigma_{\Theta}(T)=\oslash\}
\end{aligned}
}$$

\leftline{12. SUM: sum($T.\beta$)\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \   13. COUNT: count($T.\beta$) }
$$\frac{
\{T,\beta\}\
}{
\begin{aligned}
    \{x_{sum} | x_{sum}=\sum_{v \in \pi_{\beta}(T)}v\}
\end{aligned}
}\ \ \ \ \ \ \ \  \frac{
\{T,\beta\}
}{
\begin{aligned}
    \{x_{count} | x_{count}=\sum_{\alpha \in T}(\xi_{\alpha} (T)) \}
\end{aligned}
}$$

% \leftline{13. COUNT: count($T.\beta$) \\ }
% $$\frac{
% \{T,\beta\}
% }{
% \begin{aligned}
%     \{x_{count} | x_{count}=\sum_{\alpha \in T}(\xi_{\alpha} (T)) \}
% \end{aligned}
% }$$

\end{framed}
\begin{framed}
\leftline {\textbf{Group operation}\\}
~\\
\leftline{14. GROUP BY: group by $T.\beta$\\ }
$$\frac{
\{T,\beta\}\
}{
\begin{aligned}
    \{T_{1}=(\overline{\beta},&(\overline{\alpha_1},...,\overline{\alpha_k})) |\forall \overline{\alpha_i} \in\ (\overline{\alpha_1},...,\overline{\alpha_k}), 
 (\forall\ v_{ij}\ \in\ \pi_{\beta}(\overline{\alpha_i}),\\&(v_{ij}=v_{i1})   
 \wedge(\forall\ v_{xy}\ \in \pi_{\beta}(\overline{\alpha_x}), 
(v_{ij}\ne v_{xy}),\\
(x\in(1,...,k)&)\wedge(x\ne i)))   
 \wedge(\forall \alpha_x \in T,\xi_{\alpha_x}(T_1)=\xi_{\alpha_x}(T))
\\
&\wedge(\forall \alpha_y \in T_1,\xi_{\alpha_y}(T_1)=\xi_{\alpha_y}(T))\}
\end{aligned}
}$$

\leftline{15. HAVING: having\ $\Theta$\\ }
$$\frac{
\{T,\Theta\}
}{
\begin{aligned}
    \{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1)& 
 \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)
\\
 \wedge(\xi_{\alpha}(T)=&\xi_{\alpha}(T_1))\}
\end{aligned}
}$$

\leftline{16. DISTINCT: distinct\ $T.\beta$ \\ }
$$\frac{
\{T,\beta\}\
}{
\begin{aligned}
    \{T_{1} | (\forall \alpha \in T,\ \xi_{\alpha} (T_1)=1) 
 \wedge(\forall \alpha_1 \in T_1,\ \alpha_1 \in T )\}
\end{aligned}
}$$

\leftline{17. ORDER BY: order by\ $T.\beta$ desc\\ }
$$\frac{
\{T,\beta\}\
}{
\begin{aligned}
    \{T_{1} | (\forall \alpha \in T_1,\ \xi_{\alpha} (T_1)=\xi_{\alpha} (T)) &
\wedge(\forall \alpha \in T,\ \xi_{\alpha} (T)=\xi_{\alpha} (T_1))\\
 \wedge(\forall \alpha_i \in \sigma_{T_1.{\overline{\beta}}}(&T_1),\ \alpha_i > \alpha_{i+1} )\}
\end{aligned}
}$$

\leftline{18. ORDER BY: order by\ $T.\beta$ asc\\ }
$$\frac{
\{T,\beta\}\
}{
\begin{aligned}
    \{T_{1} | (\forall \alpha \in T_1,\ \xi_{\alpha} (T_1)=\xi_{\alpha} (T)) &
\wedge(\forall \alpha \in T,\ \xi_{\alpha} (T)=\xi_{\alpha} (T_1))\\
 \wedge(\forall \alpha_i \in \sigma_{T_1.{\overline{\beta}}}(&T_1),\ \alpha_i < \alpha_{i+1} )\}
\end{aligned}
}$$
\end{framed}
\begin{framed}
\leftline {\textbf{Condition}\\}
~\\

\leftline{18. EXISTS:  exists($\Theta$)\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  19.  AND:  $\Theta_1$\ and\ $\Theta_2$ \\ }
$$\frac{
\{\Theta \}
}{
\begin{aligned}
    \{\Theta_1 | \Theta_1=(\Theta = TRUE)\}
\end{aligned}
}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
\frac{
\{\Theta_{1}, \Theta_{2}\}
}{
\begin{aligned}
    \{\Theta |  \Theta=\Theta_{1} \wedge \Theta_{2} \}
\end{aligned}
}
$$

% \leftline{19.  AND:  $\Theta_1$\ and\ $\Theta_2$ \\ }
% $$\frac{
% \{\Theta_{1}, \Theta_{2}\}
% }{
% \begin{aligned}
%     \{\Theta |  \Theta=\Theta_{1} \wedge \Theta_{2} \}
% \end{aligned}
% }$$

\leftline{20. OR:  $\Theta_1$\ or\ $\Theta_2$\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  21. NOT:  not $\Theta$\\ }
$$\frac{
\{\Theta_{1}, \Theta_{2}\}
}{
\begin{aligned}
    \{\Theta |  \Theta=\Theta_{1} \vee \Theta_{2} \}
\end{aligned}
}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
\frac{
\{\Theta_{1}\}
}{
\begin{aligned}
    \{\Theta |  \Theta = \neg \Theta_{1}\}
\end{aligned}
}
$$
% \leftline{21. NOT:  not $\Theta$ \\ }
% $$\frac{
% \{\Theta_{1}\}
% }{
% \begin{aligned}
%     \{\Theta |  \Theta = \neg \Theta_{1}\}
% \end{aligned}
% }$$


\leftline{22. $\Theta$ IS NULL:  $\Theta$ is null\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 23. $\Theta$ IS NOT NULL:  $\Theta$ is not null \\ }
$$\frac{
\{\Theta\}\
}{
\begin{aligned}
    \{\Theta_1 |  \Theta_1 = (\Theta\ =\ NULL)\}
\end{aligned}
}\ \ \ \ \ \ \ \frac{
\{\Theta\}\
}{
\begin{aligned}
    \{\Theta_1 |  \Theta_1 = (\Theta\ \ne\ NULL)\}
\end{aligned}
}$$
% \leftline{23. $\Theta$ IS NOT NULL:  $\Theta$ is not null \\ }
% $$\frac{
% \{\Theta\}\
% }{
% \begin{aligned}
%     \{\Theta_1 |  \Theta_1 = (\Theta\ \ne\ NULL)\}
% \end{aligned}
% }$$
\leftline{17. BETWEEN: between value1 and value2 \\ }
$$\frac{
\{T,\beta,value_1,value_2\}\
}{
\begin{aligned}
    \{\Theta |  \Theta=(v \in \pi_{\beta}(T), \}
(v \ge value1) \wedge (v \le value2))\}
\end{aligned}
}$$
\end{framed}
\begin{framed}
\leftline {\textbf{Join operation}\\}
~\\
\leftline{24. NATURAL JOIN :  $T_1$ natural join $T_2$ \\ }
$$\frac{
\{T_{1}, T_{2}\}
}{
\begin{aligned}
    &\{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta}))
\\
 \wedge(\forall \alpha_1 &\in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))\\ 
\wedge(\forall \alpha_2 &\in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
}$$
\leftline{25. LEFT JOIN :  $T_1$ left join $T_2$\\ }
$$\frac{
\{T_{1}, T_{2}\}
}{
\begin{aligned}
    \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee((\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta})))
\\
 \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))\\ 
\wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
}$$
\leftline{26. RIGHT JOIN :  $T_1$ right join $T_2$ \\ }
$$\frac{
\{T_{1}, T_{2}\}
}{
\begin{aligned}
    \{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_2.\overline{\beta})\vee((\beta \in T_1.\overline{\beta})\wedge(\beta \in T_2.\overline{\beta})))
\\
 \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))\\ 
\wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
}$$
\leftline{27. FULL JOIN :  $T_1$ full join $T_2$ \\ }
$$\frac{
\{T_{1}, T_{2}\}
}{
\begin{aligned}
    &\{T | (\forall \beta \in T.\overline{\beta},(\beta \in T_1.\overline{\beta})\vee(\beta \in T_2.\overline{\beta}))
\\
 \wedge(\forall \alpha_1 &\in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1),\xi_{\alpha_1}(T)=\xi_{\alpha_1}(T_1))\\ 
\wedge(\forall \alpha_2 &\in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2),\xi_{\alpha_2}(T)=\xi_{\alpha_2}(T_2)) \}
\end{aligned}
}$$
\leftline{15. ON: on\ $\Theta$\\ }
$$\frac{
\{T,\Theta\}
}{
\begin{aligned}
    \{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1) &
 \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)
\\
 \wedge(\xi_{\alpha}(T)=&\xi_{\alpha}(T_1))\}
\end{aligned}
}$$
\end{framed}
\begin{framed}
\leftline {\textbf{String Function}\\}
~\\
\leftline{25. RTRIM :  rtrim($str$) \\ }
$$\frac{
\{str\}
}{
\begin{aligned}
    \{str1 | (str1=str&[0,len(str1)])\\ 
 \wedge(\forall i \in (len(str1),len(&str)),str[i]=space) \}
\end{aligned}
}$$

\leftline{26. LTRIM :  ltrim($str$) \\ }
$$\frac{
\{str\}
}{
\begin{aligned}
    \{str1 | (str1=str[len(str)-len(str1),len(str)])\\
 \wedge(\forall i \in (0,len(str)-len(str1)),str[i]=space) \}
\end{aligned}
}$$

\leftline{27. RPAD :  rpad($str,length,str1$) \\ }
$$\frac{
\{str,length,str1\}
}{
\begin{aligned}
    \{&str2 | (len(str2)=length)
\wedge(str2[0,len(str)]=str)
 \wedge\\
 (\forall i &\in (len(str),len(str2),
str2[i]=str1[(i-len(str))\%(str1)]) \}
\end{aligned}
}$$

\leftline{28. LPAD :  lpad($str,length,str1$) \\ }
$$\frac{
\{str,length,str1\}
}{
\begin{aligned}
    \{str2 | (len(str2)=length) 
 \wedge(str2[len(str2)-len(str),len(str2)]\\
 =str) 
\wedge(\forall i \in (0,len(str2)-len(str),
str2[i]=str1[i\%len(str1)]) \}
\end{aligned}
}$$

\leftline{29. RIGHT :  right($str,length$) \\ }
$$\frac{
\{str,length\}
}{
\begin{aligned}
    \{str1 | str1=str[len(str)-length,len(str)] \}
\end{aligned}
}$$

\leftline{30. LEFT :  left($str,length$) \\ }
$$\frac{
\{str,length\}
}{
\begin{aligned}
    \{str1 | str1=str[0,length]\}
\end{aligned}
}$$

\leftline{31. INSTR :  instr($str1,str2$) \\ }
$$\frac{
\{str1,str2\}
}{
\begin{aligned}
    \{n | str2=str1[&n,n+len(str2)]\\
 \wedge(\forall i \in (0,n-1),str1[i,&i+len(str2)]\ne str2\}
\end{aligned}
}$$

\leftline{32. LOCATE POSITION :locate/position($str1,str2,start$)\\} 
% \leftline{locate/position($str1,str2,start$) \\}
$$\frac{
\{str1,str2,start\}
}{
\begin{aligned}
    \{n | str1=str2[&n,n+len(str1)]\\ 
\wedge(\forall i \in (start,n),str2[&i,i+len(str1)]\ne str1\}
\end{aligned}
}$$

\leftline{33. SUBSTR SUBSTRING MID :substr/substring/mid($str,start,length$)\\} 
% \leftline{substr/substring/mid($str,start,length$) \\ }
$$\frac{
\{str,start,length\}
}{
\begin{aligned}
    \{str1 | str1=str[sta&rt,start+length]\} \\
\wedge(\forall i \in (start,n),str2[i,&i+len(str1)]\ne str1\}
\end{aligned}
}$$

\leftline{34. SUBSTRING_INDEX :substring_index($str,char,index$)\\} 
% \leftline{substring_index($str,char,index$) \\ }
$$\frac{
\{str,char,index\}
}{
\begin{aligned}
    \{str1 | str1=str[0,len(str1)]& 
 \wedge(str[len(str1)]=index \\
\wedge(\xi_{char}(str)&=index-1\}\\
\end{aligned}
}$$

\leftline{35. REVERSE :  reverse($str$) \\ }
$$\frac{
\{str\}
}{
\begin{aligned}
    \{str1 | (len(st&r1)=len(str))\\
 \wedge(\forall i \in (0,len(str)),str[i]&=str1[len(str1)-i])\}
\end{aligned}
}$$

\leftline{36. INSERT :  insert($str,start,length,str1$) \\ }
$$\frac{
\{str,start,length,str1\}
}{
\begin{aligned}
    \{str2 | (str2[0,start]=str[0,start]) 
\wedge
(str2[start+len(str1),\\
len(str2)]
=str[start+length,len(str2)])
\wedge(str2[,start,start+\\
len(str1)]=str1
\wedge(len(str2)-len(str1=len(str)-length)\}
\end{aligned}
}$$

\leftline{37. FIND\_IN\_SET FIELD :  find\_in\_set/field($str,\overline{str}$) \\ }
$$\frac{
\{str,\overline{str}\}
}{
\begin{aligned}
    \{n | (\overline{str}[n]=str) 
\wedge(\forall i \in (0,n),\overline{str} \ne str)\}
\end{aligned}
}$$

\leftline{38. ELT :  elt($index,\overline{str}$) \\ }
$$\frac{
\{index,\overline{str}\}
}{
\begin{aligned}
    \{str | (\overline{str}[index]=str)
\wedge(\forall i \in (0,index),\overline{str}[i]\ne str)\}
\end{aligned}
}$$

\leftline{39. SPACE :  space($n$) \\ }
$$\frac{
\{n\}
}{
\begin{aligned}
    \{str | (len(str)=n)\wedge(\forall i \in (0,len(str)),str[i]=space)\}
\end{aligned}
}$$

\leftline{40. REPEAT :  repeat($str,n$) \\ }
$$\frac{
\{str,n\}
}{
\begin{aligned}
    \{str1 | (len(str1)&=n*len(str))\\ 
\wedge(\forall i \in (0,len(str1)),str1&[i]=str[i\%len(str)])\}
\end{aligned}
}$$

\leftline{41. UPPER UCASE :  upper/ucase($str$) \\ }
$$\frac{
\{str\}
}{
\begin{aligned}
    \{str | (len(str)&=len(str1))\\ 
 \wedge(\forall i \in (0,len(str)),str1[&i]=ascii(str[i]-32))\}
\end{aligned}
}$$

\leftline{42. LOWER LCASE :  lower/lcase($str$) \\ }
$$\frac{
\{str\}
}{
\begin{aligned}
    \{str | (len(str)&=len(str1))\\ 
 \wedge(\forall i \in (0,len(str)),str1[&i]=ascii(str[i]+32))\}
\end{aligned}
}$$

\leftline{43. ASCII :  ascii($char$)\ \ \ \ \ \ \ \ \ \ \ \ \ \  44. CHAR :  char($n$) \\ }
$$\frac{
\{char\}
}{
\begin{aligned}
   \{n | n=char+0\} 
\end{aligned}
}\ \ \ \ \ \ \ \ \ \ \ \ 
\frac{
\{n\}
}{
\begin{aligned}
    \{char | char=ascii(n)\}
\end{aligned}
}$$

\leftline{44. CHAR :  char($n$) \\ }
$$\frac{
\{n\}
}{
\begin{aligned}
    \{char | char=ascii(n)\}
\end{aligned}
}$$

\leftline{45. CASE IF :  case when $\Theta$ then $\Theta_{1}$ else $\Theta_{2}$/if($\Theta,\Theta_{1},\Theta_{2}$) \\ }
$$\frac{
\{\Theta,\Theta_{1},\Theta_{2}\}
}{
\begin{aligned}
    \{\Theta_{3} | \Theta_{3}=\Theta_{1}, \Theta=TRUE;
\Theta_{3}=\Theta_{2}, \Theta=FALSE\}
\end{aligned}
}$$

\leftline{46. NULLIF :  nullif($\Theta_{1},\Theta_{2}$) \\ }
$$\frac{
\{\Theta_{1},\Theta_{2}\}
}{
\begin{aligned}
    \{\Theta_{3} | \Theta_{3}=NULL, \Theta_{1}=\Theta_{2}; 
\Theta_{3}=\Theta_{1}, \Theta_{1}\ne \Theta_{2} \}
\end{aligned}
}$$

\leftline{47. COALESCE :  coalesce($\overline{str}$) \\ }
$$\frac{
\{\overline{str}\}
}{
\begin{aligned}
    \{n | (\overline{str}[n]=NULL) 
\wedge(\forall i \in (0,n),\overline{str}\ne NULL)\}
\end{aligned}
}$$
\end{framed}
}

%在关键字语义的基础上，我们给出了四种常见语句模式的组合语义，这些组合语义包含的关键字有select，from，where，group by，order by，having，聚合函数

\leftline {\textbf{Compound semantics}\\}Building upon the foundation of keyword semantics, we have provided composite semantics for four common statement patterns. These composite semantics encompass keywords such as select, from, where, group by, order by, having, and aggregate functions.
{\scriptsize
\begin{framed}
\leftline {\textbf{Query expression}\\}
\leftline{$ T_s:\left\{\pi_{\overline{\beta}}(T)\right\}$}
~\\
\leftline{$ T_w:\left\{(\forall \alpha \in \sigma_\Theta (T),\alpha \in T_w)\\ \right.$}
\leftline{$\left. \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_w)\right.$}
\\
\leftline{$\left. \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_w))\right\}$}
\\ \hspace*{\fill} \\
\leftline{$ T_{sw}:\left\{\pi_{\overline{\beta}}(T_s)\right\}$}
\\ \hspace*{\fill} \\
\leftline{1. SELECT $T.\overline{\beta}$ FROM T \\ }
\\ \hspace*{\fill} \\
$\frac{\left\{T\right\}\ FROM\ \left\{T\right\},\ \left\{T\right\}\ SELECT\ \overline{\beta}\  \left\{T_{s}\right\}}{\left\{T\right\}\ FROM;\ SELECT\ \overline{\beta}   \left\{T_{s}\right\}}$
\\ \hspace*{\fill} \\
~\\
\leftline{2. SELECT $T.\overline{\beta}$ FROM T WHERE $\Theta$ \\ }
\\ \hspace*{\fill} \\
$\frac{\left\{T\right\}\ FROM\ \left\{T\right\},\ \left\{T\right\}\ WHERE\ \Theta\  \left\{T_w\right\},\left\{T_w\right\}\ SELECT\ \overline{\beta}\   \left\{T_{sw}\right\}}{\left\{T\right\}\ FROM;\ WHERE\ \Theta;\ SELECT\ \overline{\beta}\    \left\{T_{sw}\right\}}$
\\ \hspace*{\fill} \\
~\\
\leftline{7. SELECT $\beta_1$, Aggregation Operation ($T.\beta_2$) FROM T \\}
\leftline{GROUP BY $\beta_1$ HAVING $\Theta$ \\ }
~\\
$\frac{\left\{T\right\}\ FROM\ \left\{T_1\right\},\ \left\{T_1\right\}\ GROUP\ BY\ \left\{T_2\right\},\ \left\{T_2,\beta_2\right\}\ Agg\ \left\{x_{agg}\right\},\ \ }{\left\{T,\beta_2\right\}\ FROM;\ GROUP\ BY;\ AGG     \left\{x_{agg}\right\}}$
\\ \hspace*{\fill} \\
$\frac{\left\{T_2,\beta_1,\beta_2,x_{agg}\right\}\ SELECT\ \left\{T_3\right\},\ \left\{T_3,\Theta\right\}\ HAVING\ \left\{T_4\right\}\ }{\left\{T_2,\beta_1,\beta_2,x_{agg}\right\}\ SELECT;\ HAVING;\     \left\{T_4\right\}}$
\\ \hspace*{\fill} \\
~\\
\leftline{7. SELECT $T.\beta_1$ FROM T ORDER BY $\beta_1$ ASC/DESC\\}
~\\
$\frac{\left\{T\right\}\ FROM\ \left\{T_1\right\},\ \left\{T_1,\beta_1\right\}\ SELECT\ \left\{T_2\right\} \ }{\left\{T,\beta_1\right\}\ FROM;\ SELECT;\left\{T\right\} }$
\\ \hspace*{\fill} \\
$\frac{\left\{T_2,\beta_1\right\}\ ORDER\ BY \left\{T_3\right\} }{\left\{T_2,\beta_1\right\}\ ORDER\ BY;\     \left\{T_3\right\}}$
\end{framed}
}
\end{spacing}
% \begin{figure*}
% \begin{framed}
% \leftline {\textbf{KEYWORD}\\}
% \leftline {\textbf{Query expression}\\}
% \leftline {1. FROM: from T\\}
% $\left\{T\right\}\ FROM\ \left\{T_1\right\}$
% \\ \hspace*{\fill} \\
% \leftline {2. SELECT: select\ $T.\overline{\beta}$\\}
% $\left\{T,\overline{\beta}\right\}\ SELECT\ \left\{T_1|T_1=\left\{\pi_{\overline{\beta}}(T)\right\}\right\}$
% \\ \hspace*{\fill} \\
% \leftline {3. WHERE: where\ $\Theta$\\}
% $\left\{T,\Theta\right\}\ WHERE$
% $\left\{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1)\\ \right.$
% $\left. \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)\right.$
% $\left. \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\right\}$
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Collection operation}\\}
% \leftline{4. UNION: T1 union T2 \\ }
% $
% \left\{T_{1}, T_{2}\right\}\ UNION$
% \\
% $\left\{T | (\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2, \alpha_{1} , \alpha_{2} \in T) \right.$
% \\
% $\left. \wedge(\forall \alpha_{3} \in T,(\alpha_{3} \in T_1)\vee(\alpha_{3} \in T_2))\right.$
% $ \left. \wedge (\forall \alpha_4 \in T,\ \xi_{\alpha_4}(T)=1)\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{5. INTERSECT: T1 intersect T2 \\ }
% $\left\{T_{1}, T_{2}\right\}\ INTERSECT$
% \\
% $
% \left\{T | (\forall \alpha_{1} \in T_1,  ((\alpha_{1}  \in T_2) \wedge (\alpha_{1}  \in T)) \right.$
% $ \left. \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \notin T_2)))\right.$
% \\
% $\left. \wedge(\forall \alpha_{2} \in T,(\alpha_{2} \in T_1)\vee(\alpha_{2} \in T_2))\right.$
% $ \left. \wedge (\forall \alpha_3 \in T,\ \xi_{\alpha_3}(T)=1)\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{6. EXCEPT: T1 except T2 \\ }
% $\left\{T_{1}, T_{2}\right\}\ EXCEPT $
% \\
% $
% \left\{T | (\forall \alpha_{1} \in T_1,  ((\alpha_{1}  \in T) \wedge (\alpha_{1}  \notin T_2) \right.$
% $ \left. \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \in T_2)))\right.$
% \\
% $\left. \wedge(\forall \alpha_{2} \in T,(\alpha_{2} \in T_1))\right.$
% $ \left. \wedge (\forall \alpha_3 \in T,\ \xi_{\alpha_3}(T)=1)\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{7. UNION ALL: T1 union all T2 \\ }
% $
% \left\{T_{1}, T_{2}\right\}\ UNION\ ALL $
% \\
% $\left\{T | (\forall \alpha_{1} \in T_1,\forall \alpha_{2} \in T_2,\right.$
% $\left. \alpha_{1} , \alpha_{2} \in T) \right.$
% \\
% $\left. \wedge(\forall \alpha_{3} \in T,(\alpha_{3} \in T_1)\vee(\alpha_{3} \in T_2))\right.$
% $ \left. \wedge (\forall \alpha_4 \in T,\ \xi_{\alpha_4}(T)=\xi_{\alpha_4}(T_1)+\xi_{\alpha_4}(T_2))\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{8. INTERSECT ALL: T1 intersect all T2 \\ }
% $\left\{T_{1}, T_{2}\right\}\ INTERSECT\ ALL $
% \\
% $
% \left\{T | (\forall \alpha_{1} \in T_1, \right.$
% $ \left.((\alpha_{1}  \in T_2) \wedge (\alpha_{1}  \in T) \right.$
% $ \left. \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \notin T_2)))\right\}$
% \\
% $ \left. \wedge (\forall \alpha_2 \in T,\ \right.$
% $\left. \xi_{\alpha_2}(T)=min(\xi_{\alpha_2}(T_1),\xi_{\alpha_2}(T_2)))\right\}
% $
% \\ \hspace*{\fill} \\
% \leftline{9. EXCEPT ALL: T1 except all T2 \\ }
% $\left\{T_{1}, T_{2}\right\}\ EXCEPT\ ALL $
% \\
% $
% \left\{T | (\forall \alpha_{1} \in T_1,\right. $
% $ \left.((\alpha_{1}  \in T) \wedge (\alpha_{1}  \notin T_2) \right.$
% $ \left. \vee ((\alpha_{1}  \notin T) \wedge (\alpha_{1}  \in T_2)))\right\}$
% \\
% $ \left. \wedge (\forall \alpha_2 \in T,\ \right.$
% $ \left. \xi_{\alpha_2}(T)=max(\xi_{\alpha_2}(T_1)-\xi_{\alpha_2}(T_2)),0)\right\}
% $
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Aggregation operation}\\}
% \leftline{10. MIN: min($T.\beta$) \\ }
% $\left\{T,\beta\right\}\ MIN $
% \\
% $\left\{
% x_{min} | (x_{min} \in \pi_{\beta}(T),
% \right. $ 
% $\left. \Theta=(v \in \pi_{\beta}(T)\wedge(v < x_{min})),\ \sigma_{\Theta}(T)=\oslash \right\} $
% \\ \hspace*{\fill} \\
% \leftline{11. MAX: max($T.\beta$) \\ }
% $\left\{T,\beta\right\}\ MAX $
% \\
% $\left\{x_{max} | x_{max} \in \pi_{\beta}(T), \right. $
% $\left.\Theta=(v \in \pi_{\beta}(T) \wedge(v > x_{max})),\ \sigma_{\Theta}(T)=\oslash\right\}$
% \end{framed}
% \end{figure*}
% \begin{figure*}
% \begin{framed}
% \leftline{12. SUM: sum($T.\beta$) \\ }
% $\left\{T,\beta\right\}\ SUM\ \left\{x_{sum} | x_{sum}=\sum_{v \in \pi_{\beta}(T)}v,\right\}$
% \\ \hspace*{\fill} \\

% \leftline{13. COUNT: count($T.\beta$) \\ }
% $\left\{T,\beta\right\}\ COUNT\ \left\{x_{count} | x_{count}=\sum_{\alpha \in T}(\xi_{\alpha} (T))  \right\}$
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Group operation}\\}
% \leftline{14. GROUP BY: group by $T.\beta$\\ }
% $\left\{T,\beta\right\}\ GROUP BY $
% \\
% $\left\{T_{1}=(\overline{\beta},(\overline{\alpha_1},...,\overline{\alpha_k})) |\forall \overline{\alpha_i} \in\ (\overline{\alpha_1},...,\overline{\alpha_k}), \right.$
% $\left. (\forall\ v_{ij}\ \in\ \pi_{\beta}(\sigma_{TRUE}(\overline{\alpha_i})),(v_{ij}=v_{i1})   \right.$
% \\
% $\left. \wedge(\forall\ v_{xy}\ \in\ \pi_{\beta}(\sigma_{TRUE}(\overline{\alpha_x})),(v_{ij}\ne v_{xy}),(x\in(1,...,k))\wedge(x\ne i)))   \right.$
% \\
% $\left. \wedge(\forall \alpha_x \in T,\xi_{\alpha_x}(T_1)=\xi_{\alpha_x}(T))\right.$
% $\left. \wedge(\forall \alpha_y \in T_1,\xi_{\alpha_y}(T_1)=\xi_{\alpha_y}(T))\right\}$
% \\ \hspace*{\fill} \\
% \leftline{15. HAVING: having\ $\Theta$\\ }
% $\left\{T,\Theta\right\}\ HAVING $
% \\
% $\left\{T_1 | (\forall \alpha \in \sigma_\Theta (T),\alpha \in T_1)\\ \right.$
% $\left. \wedge(\forall \alpha_1 \notin \sigma_{\Theta} (T),\alpha_1 \notin T_1)\right.$
% $\left. \wedge(\xi_{\alpha}(T)=\xi_{\alpha}(T_1))\right\}$
% \\ \hspace*{\fill} \\
% \leftline{16. DISTINCT: distinct\ $T.\beta$ \\ }
% $\left\{T,\beta\right\}\ DISTINCT $
% \\
% $\left\{T_{1} | (\forall \alpha \in T,\ \xi_{\alpha} (T_1)=1) \right.$
% $\left. \wedge(\forall \alpha_1 \in T_1,\ \alpha_1 \in T )\right\}$
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Condition}\\}
% \leftline{17. BETWEEN: between value1 and value2 \\ }
% $\left\{T,\beta,value_1,value_2\right\}\ BETWEEN $
% \\
% $\left\{\Theta |  \Theta=(v \in \pi_{\beta}(T), (v \ge value1) \wedge (v \le value2))\right\}$
% \\ \hspace*{\fill} \\
% \leftline{18. EXISTS:  exists($\Theta$) \\ }
% $\left\{\Theta \right\}\ EXISTS\ \left\{\Theta_1 | \Theta_1=(\Theta = TRUE)\right\}$
% \\ \hspace*{\fill} \\
% \leftline{19.  AND:  $\Theta_1$\ and\ $\Theta_2$ \\ }
% $\left\{\Theta_{1}, \Theta_{2}\right\}\ AND\ \left\{\Theta |  \Theta=\Theta_{1} \wedge \Theta_{2} \right\}$
% \\ \hspace*{\fill} \\
% \leftline{20. OR:  $\Theta_1$\ or\ $\Theta_2$ \\ }
% $\left\{\Theta_{1}, \Theta_{2}\right\}\ OR\ \left\{\Theta |  \Theta=\Theta_{1} \vee \Theta_{2} \right\}$
% \\ \hspace*{\fill} \\
% \leftline{21. NOT:  not $\Theta$ \\ }
% $\left\{\Theta_{1}\right\}\ NOT\ \left\{\Theta |  \Theta = \neg \Theta_{1}\right\}$
% \\ \hspace*{\fill} \\
% \leftline{22. t IS NULL:  t is null \\ }
% $\left\{t\right\}\ IS\ NULL\ \left\{\Theta |  \Theta = (t\ =\ NULL)\right\}$
% \\ \hspace*{\fill} \\
% \leftline{23. t IS NOT NULL:  t is not null \\ }
% $\left\{t\right\}\ IS\ NOT\ NULL\ \left\{\Theta |  \Theta = (t\ \ne\ NULL)\right\}$
% \end{framed}
% \begin{framed}
% \leftline {\textbf{Join operation}\\}
% \leftline{24. NATURAL JOIN :  $T_1$ natural join $T_2$ \\ }
% $\left\{T_{1}, T_{2}\right\}\left\{NATURAL\ JOIN\right\}$
% \\
% $\left\{T | (\forall \beta_1 \in T_1.\overline{\beta},\beta_1 \in T.\overline{\beta},\xi_{\beta_1}(T)=1;\\ \right.$
% $\left. \forall \beta_2 \in T_2.\overline{\beta},\beta_2 \in T.\overline{\beta},\xi_{\beta_2}(T)=1;\right.)$
% \\
% $
% \left. \wedge(\forall \alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T),\alpha_1 \in \sigma_{T_1.{\overline{\beta}}}(T_1))\\ \right.$
% $
% \left. \wedge(\forall \alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T),\alpha_2 \in \sigma_{T_2.{\overline{\beta}}}(T_2)) \right\}$
% \end{framed}
% \end{figure*}






==> wenfa.tex <==
\begin{figure*}[t]
\begin{framed}
% \leftline{
% $
% (1)\langle queryexp\rangle       ::= \langle select\ clause\rangle       \langle from\ clause\rangle
% $}
% \leftline{$(2)\langle select\ clause\rangle       ::= select      \ \langle slist\rangle       $}
% \leftline{$(3)\langle slist\rangle       ::= * | \langle cname\rangle      \ [ {,\ \langle cname\rangle       }... ]$}
% \leftline{$(4)\langle from\ clause\rangle       ::= from \langle tref\rangle       [ { , \langle tref\rangle       }... ]  $}
% \leftline{$(5)\langle tref\rangle       ::= \langle tname\rangle\ |\ \langle joined\ table\rangle         $}
% \leftline{$(6)\langle joined\ table\rangle       ::= \langle cross\ join\rangle\ |\ \langle qualified\ join\rangle\ |\ \langle natural\ join\rangle       $}
% \leftline{$(7)\langle cross\ join\rangle       ::= \langle tname\rangle       cross\ join \langle tname\rangle       $}
% \leftline{$(8)\langle qualified\ join\rangle       ::= \langle tname\rangle         [ inner |  left | right | full]\ join\langle tname\rangle \langle on\ clause\rangle     $}
% % \leftline{$\ \ \ \ \ \langle on\ clause\rangle      $}
% \leftline{$(9)\langle natural\ join\rangle       ::=\langle tname\rangle        natural\ join\  \langle tname\rangle      $}
% \leftline{$(10)\langle on\ clause\rangle       ::= on\ \langle bvexp\rangle      $}
% \leftline{$
% \begin{aligned}
% (11)\langle vexp\rangle       ::= \langle nvexp\rangle\ |\ \langle bvexp\rangle
% \end{aligned}
% $}
% \leftline{$
% \begin{aligned}
% (12)\langle bvexp\rangle       ::= \langle logical\ expression\rangle\ |\ true\ |\ false\ |\ null
% \end{aligned}
% $}
% \leftline{$
% \begin{aligned}
% (13)\langle logical\ expression\rangle       ::= \langle bvexp\rangle\       OR\ \langle bvexp\rangle\ |\ \langle bvexp\rangle\ AND\ \langle bvexp\rangle\ |\ \langle bvexp\rangle\       XOR\langle bvexp\rangle\       | NOT\ \langle bvexp\rangle 
% \end{aligned}
% $}
% % \leftline{$
% % \begin{aligned}
% % \ \ \ \ \ \langle bvexp\rangle\ |\ \langle bvexp\rangle\       XOR\langle vexp\rangle\       | NOT\ \langle vexp\rangle      
% % \end{aligned}
% % $}
% \leftline{$
% (14)\langle nvexp\rangle       ::= \langle arithmetic\ expression\rangle\ |\ numeric\ literal
% $}
% \leftline{$
% (15)\langle arithmetic\ expression\rangle       ::= \langle nvexp\rangle       + \langle nvexp\rangle\        |\ \langle nvexp\rangle       - \langle nvexp\rangle\ |\ \langle nvexp\rangle       * \langle nvexp\ \rangle\ |\ \langle nvexp\rangle       / \langle nvexp\ \rangle
% $}
% \leftline{$(16)\langle tname\rangle       ::= identifier       $}
% \leftline{$(17)\langle cname\rangle       ::= identifier       $}

% \leftline{$(3)\langle table\ reference\rangle       ::= \langle table\ name\rangle      $ }
% \leftline{$(4)\langle column\ reference\rangle       ::= \langle table\ name\rangle      .\langle column\ name\rangle       $ }
% \leftline{$(5)\langle literal\rangle       ::=  \langle numeric\ literal\rangle\ |\ \langle string\ literal\rangle\ |\ \langle boolean\ literal\rangle\ |\ \langle null\rangle      $}
% \leftline{$(6)\langle data\ type\rangle       ::= \langle string\ type\rangle\ |\ \langle numeric\ type\rangle\ |\ \langle boolean\ type\rangle      
% $}

\leftline{$
(1)\langle queryexp\rangle       ::= \{\ \langle select\ clause\rangle       \langle from\ clause\rangle  [ \langle where\ clause\rangle       ][ \langle group\ by\ clause\rangle       ]     
$}

\leftline{$
\ \ \ \ \ [ \langle having\ clause\rangle       ]\} [ \langle order\ by\ clause\rangle       ]
$}

\leftline{$(4)\langle from\ clause\rangle       ::= FROM \langle tref\rangle       [ { , \langle tref\rangle       }... ]  $}
\leftline{$(5)\langle tref\rangle       ::= \langle tname\rangle\ |\ \langle joined\ table\rangle         $}
\leftline{$(6)\langle joined\ table\rangle       ::= \ \langle natural\ join\rangle\ |\ cross\ join       $}
\leftline{$(9)\langle natural\ join\rangle       ::=\langle tname\rangle        NATURAL\ JOIN\  \langle tname\rangle      $}
\leftline{$(11)\langle where\ clause\rangle       ::= WHERE \langle bvexp\rangle        $}

% \leftline{\textbf{SELECT操作}}

\leftline{$(12)\langle select\ clause\rangle       ::= SELECT\ \langle sop\rangle      \ \langle slist\rangle       $}
\leftline{$(13)\langle slist\rangle       ::= * | \langle cname\rangle      \ [ {,\ \langle cname\rangle       }... ]$}
\leftline{$(14)\langle sop\rangle       ::= DISTINCT\ | ALL\ $}

% \leftline{\textbf{GROUP BY操作}}

\leftline{$(16)\langle group\ by\ clause\rangle       ::= GROUP\ BY\  \langle cname\rangle      $}

% \leftline{\textbf{HAVING操作}}

\leftline{$(17)\langle having\ clause\rangle       ::= HAVING \langle bvexp\rangle        $}

% \leftline{\textbf{ORDER BY操作}}

\leftline{$(18)\langle order\ by\ clause\rangle       ::= ORDER\ BY \langle cname\rangle        ASC | DESC$}
\leftline{$
\begin{aligned}
(19)\langle vexp\rangle       ::= \langle nvexp\rangle\ |\ \langle bvexp\rangle\ |\  \langle cname\rangle\ |\ null
\end{aligned}
$}
% \leftline{$
% \begin{aligned}
% \ \ \ \ \ \langle bvexp\rangle\ |\ \langle bvexp\rangle\       XOR\langle vexp\rangle\       | NOT\ \langle vexp\rangle      
% \end{aligned}
% $}
 \leftline{$
(25)\langle nvexp\rangle       ::= \langle arithmetic\ expression\rangle\ |\ \langle cname\rangle\ |\ numeric\ literal
$}
\leftline{$
(26)\langle arithmetic\ expression\rangle       ::= \langle nvexp\rangle       + \langle nvexp\rangle\        |\ \langle nvexp\rangle       - \langle nvexp\rangle\ |\ \langle nvexp\rangle       * \langle nvexp\ \rangle |\ \langle nvexp\rangle       / \langle nvexp\rangle
$}
\leftline{$
\begin{aligned}
(37)\langle bvexp\rangle       ::= \langle logical\ expression\rangle\ |\ \langle cname\rangle\ |\ true\ |\ false\ |\ null
\end{aligned}
$}
\leftline{$
\begin{aligned}
(38)\langle logical\ expression\rangle       ::= \langle bvexp\rangle\       OR\ \langle bvexp\rangle\ |\ \langle bvexp\rangle\ AND\ \langle bvexp\rangle\ |\ \langle bvexp\rangle\       XOR\langle bvexp\rangle\       | NOT\ \langle bvexp\rangle 
\end{aligned}
$}
\leftline{$(50)\langle tname\rangle       ::= identifier       $}
\leftline{$(51)\langle cname\rangle       ::= identifier       $}
\end{framed}
\caption{Selected grammar for SQL}
\label{fig:wenfa}
\end{figure*}
